Status-quo policy gradient in Multi-Agent Reinforcement Learning

Individual rationality, which involves maximizing expected individual returns, does not always lead to high-utility individual or group outcomes in multi-agent problems. For instance, in multi-agent social dilemmas, Reinforcement Learning (RL) agents trained to maximize individual rewards converge to a low-utility mutually harmful equilibrium. In contrast, humans evolve useful strategies in such social dilemmas. Inspired by ideas from human psychology that attribute this behavior to the status-quo bias, we present a status-quo loss (SQLoss) and the corresponding policy gradient algorithm that incorporates this bias in an RL agent. We demonstrate that agents trained with SQLoss learn high-utility policies in several social dilemma matrix games (Prisoner's Dilemma, Stag Hunt matrix variant, Chicken Game). We show how SQLoss outperforms existing state-of-the-art methods to obtain high-utility policies in visual input non-matrix games (Coin Game and Stag Hunt visual input variant) using pre-trained cooperation and defection oracles. Finally, we show that SQLoss extends to a 4-agent setting by demonstrating the emergence of cooperative behavior in the popular Braess' paradox.

==> introduction_EXPERIMENTAL.tex <==
\section{Introduction}
\label{sec:introduction}
\begin{comment}
\begin{figure}[ht]
    \includegraphics[width=\linewidth]{images/overall_idea.png}
    \caption{A schematic diagram of the proposed idea}
    \label{fig:overall_idea}
\end{figure}
\end{comment}
% In intertemporal social dilemmas, there is a tradeoff between short-term individual incentives and long-term collective interest. Humans face such dilemmas when contributing to a collective food storage during the summer in preparation for a harsh winter, organizing annual maintenance of irrigation systems, or sustainably sharing a local fishery. Classical models of human behavior based on rational choice theory predict that cooperation in these situations is impossible [1, 2]. This poses a puzzle since humans evidently do find ways to cooperate in many everyday intertemporal social dilemmas, as documented by decades of fieldwork [3, 4] and laboratory experiments [5, 6]. Providing an empirically grounded explanation of how individual behavior gives rise to societal cooperation is seen as a core goal in several subfields of the social sciences and evolutionary biology [7, 8, 9].[10, 11] proposed influential models based on behavioral game theory. However, these models have limited applicability since they only generate predictions when the problem can be cast as a matrix game (see e.g. [12, 13]). Here we consider a more realistic video-game setting, like those introduced in the behavioral research of [14, 15, 16]. In this environment, agents do not simply choose to cooperate or defect like they do in matrix games. Rather they must learn policies to implement their strategic decisions, and must do so while coping with the non-stationarity arising from other agents learning simultaneously. Several papers used multi-agent reinforcement learning [17, 18, 19] and planning [20, 21, 22, 23] to generate cooperation in this setting. However, this approach has not yet demonstrated robust cooperation in games with more than two players, which is often observed in human behavioral experiments. Moreover naïvely optimizing group reward is also ineffective, due to the lazy agent problem [24].
%It is difficult for both natural and artificial agents to find cooperative solutions to intertemporal social dilemmas for the following reasons:
%1. Collective action – individuals must learn and coordinate policies at a group level to avoid falling into socially deficient equilibria.
%2. Temporal credit assignment – rational defection in the short-term must become associated with long-term negative consequences.
%Many different research traditions, including economics, evolutionary biology, sociology, psychology, and political philosophy have all converged on the idea that fairness norms are involved in resolving social dilemmas [25, 26, 27, 28, 29, 30, 31]. In one well-known model, agents are assumed to have inequity-averse preferences [10]. They balance their selfish desire for individual rewards against a need to keep deviations between their own rewards and the rewards of others as small as possible. Inequity-averse individuals are able to solve social dilemmas by resisting the temptation to pull ahead of others or—if punishment is possible—by punishing and discouraging free-riding. The inequityaversion model has been successfully applied to explain human behavior in a variety of laboratory economic games, such as the ultimatum game, the dictator game, the gift exchange game, market games, the trust game and public goods

%Google paper
% Social dilemmas expose tensions between collective and individual rationality [1]. Cooperation makes possible better outcomes for all than any could obtain on their own. However, the lure of free riding and other such parasitic strategies implies a tragedy of the commons that thrickens the stability of any cooperative venture [2]. 
%The theory of repicked general-sum matrix games provides a framework for understanding social dilemmas. Fig. 1 shows payoff matrices for three canonical examples: Prisoner's Dilemma, Chicken, and Stag Hunt. The two actions are interpreted as cooperate and defect respectively. The four possible outcomes of each stage game are R (reward of mutual cooperation), P (punishment arising from mutual defection), S (sucker outcome obtained by the player who cooperates with a defecting partner), and T (temptation outcome achieved by defecting against a cooperator).
%A matrix game is a social dilemma when its four payoffs satisfy the following social dilemma inequalities (this formulation from [3]):
%1. R > P Mutual cooperation is preferred to mutual defection. (1)
%2. R > S Mutual cooperation is preferred to being exploited by a defector. (2)
%3. 2R > T +S This ensures that mutual cooperation is preferred to an equal probability of unilateral cooperation and defection. (3)
%4. either greed: T > R Exploiting a cooperator is preferred over mutual cooperation or fear: P > S Mutual defection is preferred over being exploited. (4)
%Matrix Game Social Dilemmas (MGSD) have been fruitfully employed as models for a wide variety of phenomena in theoretical social science and biology.


% \textcolor{red}{http://www.ifaamas.org/Proceedings/aamas2019/pdfs/p1877.pdf}
\changed{
Consider the Coin Game (\cite{asdas}, described in Figure 1).
RL agents trained to optimize individual rewards in this game learn to target 
}
\changed{There are several different approaches for extending single agent RL algorithms to multi-agent systems [Refer: Busoniu, MADDPG, COMA and some other recent MARL papers including https://arxiv.org/abs/1810.05587]. These approaches are motivated by one of five agendas---computational, descriptive, normative, prescriptive-cooperative, prescriptive-non-cooperative have been proposed for multi-agent learning (http://www.dklevine.com/archive/refs4122247000000001156.pdf).
% The computational and normative agendas deal with existence and computation of equilibria and other game theoretic solution concepts. 
The descriptive and prescriptive agendas deal with explaining agent behavior and prescribing agent behavior respectively and are most relevant for multi-agent RL problems.
Most of the recent works on MARL focus on the prescriptive agendas, which specify algorithms that agents should use to determine their policies.  In this paper, we focus on the descriptive agenda, wherein we propose an algorithm that produces outcomes that are consistent with observed human behavior in a class of games.}

\changed{MARL algorithms can be validated from the prescriptive or descriptive agendas, using some standard games, where either optimal behavior or human behavior is known. Since multi-agent systems exhibit diverse characteristics, a single algorithm is not expected to perform well in all situations. Hence, we select a specific set of games to evaluate specific aspects of an algorithm. For example, sequential social dilemmas are well-studied games, where naive extension of single-agent RL algorithms leads to a sub-optimal (both from individual and group perspectives) mutual defection outcome. Hence, they form an interesting set of problems from a prescriptive agenda perspective, as has been studied in [LOLA etc], for designing algorithms that can learn to reach the individual and socially optimal mutual cooperation solution. Sequential social dilemmas are also interesting from a descriptive agenda perspective. It has been observed in literature that humans playing sequential social dilemmas also reach the mutual cooperation solution [Ref]. Status-quo bias has been identified as one possible mechanism that leads to this outcome [REF]. In [REF], the authors provide a switching-cost based mechanism to incorporate status-quo bias in human decision making and demonstrate that this bias alone suffices prediction of the mutual cooperation outcome.  In this paper, we propose an alternate status-quo loss to incorporate status-quo bias in MARL. Our approach extends the single agent policy gradient based RL algorithm by providing an additive term that rewards preserving status-quo. We highlight two points that support the validity of this approach. The first is that this approach is a straightforward implementation of the status-quo bias from behavioral economics literature [REF] and the second is that, in numerical experiments in sequential social dilemmas, this approach yields the expected mutual cooperation outcome.}

\changed{As discussed, we choose sequential social dilemmas to illustrate the performance of our $SQLoss$ algorithm, and in the sequel we restrict attention to this class of games.} In these games, individually rational behavior leads to outcomes that are sub-optimal for each individual in the group \cite{Hardin1968,ostrom:1990,Ostrom278,Dietz1907}. Current state-of-the-art Multi-Agent Deep Reinforcement Learning (MARL) methods that train agents independently can lead to agents that fail to cooperate reliably, even in simple social dilemma settings. This failure to cooperate results in sub-optimal individual and group outcomes (\citet{foerster2018learning, Peysakhovich1707.01068}, Section~\ref{sec:approach:selfish-learner}). 

% To illustrate why it is challenging to evolve cooperation in such dilemmas, we consider the Coin Game (\citet{foerster2018learning}, Figure~\ref{fig:coin_game}). Each agent can play either selfishly (pick all coins) or cooperatively (pick only coins of its color). Regardless of the behavior of the other agent, the individually rational choice for an agent is to play selfishly, either to minimize losses (avoid being exploited) or to maximize gains (exploit the other agent). However, when both agents behave rationally, they try to pick all coins and achieve an average long term reward of $-0.5$. In contrast, if both play cooperatively, then the average long term reward for each agent is $0.5$. Therefore, when agents cooperate, they are both better off. Training Deep RL agents independently in the Coin Game using state-of-the-art methods leads to mutually harmful selfish behavior (Section~\ref{sec:approach:selfish-learner}).

The problem of how independently learning agents evolve cooperative behavior in social dilemmas has been studied by researchers through human studies and simulation models~\cite{Fudenberg, Edward:1984, Fudenberg:1984, Kamada:2010, Abreu:1990}. A large body of work has looked at the mechanism of evolution of cooperation through reciprocal behaviour and indirect reciprocity~\cite{reciprocal1971,reciprocal1984,reciprocal1992,reciprocal1993,in_reciprocal1998}, through variants of reinforcement using aspiration~\cite{reinforce_variant}, attitude~\cite{NonRL_attitude} or multi-agent reinforcement learning~\cite{Sandholm1996MultiagentRL,Wunder:2010}, and under specific conditions~\cite{R_plus_S_g_2P} using different learning rates \cite{deCote:2006} similar to WoLF~\cite{WOLF2002} as well as using embedded emotion~\cite{Emotional_Multiagent}, social networks~\cite{Ohtsuki2006,Santos:2006}.

However, these approaches do not directly apply to Deep RL agents~\cite{Leibo:2017}. Recent work in this direction~\cite{kleiman2016coordinate,Julien:2017,consequentialist18} focuses on letting agents learn strategies in multi-agent settings through interactions with other agents. \citet{Leibo:2017} define the problem of social dilemmas in the Deep RL framework and analyze the outcomes of a fruit-gathering game~\cite{Julien:2017}. They vary the abundance of resources and the cost of conflict in the fruit environment to generate degrees of cooperation between agents. \citet{Hughes:2018} define an intrinsic reward (inequality aversion) that attempts to reduce the difference in obtained rewards between agents. The agents are designed to have an aversion to both advantageous (guilt) and disadvantageous (unfairness) reward allocation. This handcrafting of loss with mutual fairness evolves cooperation, but it leaves the agent vulnerable to exploitation. LOLA~\cite{foerster2018learning} uses opponent awareness to achieve high levels of cooperation in the Coin Game and the Iterated Prisoner's Dilemma game. However, the LOLA agent assumes access to the other agent's network, observations and learning algorithms.  This level of access is analogous to getting complete access to the other agent's private information and therefore devising a strategy with full knowledge of how they are going to play.  \citet{Wang:2019} propose an evolutionary Deep RL setup to evolve cooperation. They define an intrinsic reward that is based on features generated from the agent's past and future rewards, and this reward is shared with other agents. They use evolution to maximize the sum of rewards among the agents and thus evolve cooperative behavior. However, sharing rewards in this indirect way enforces cooperation rather than evolving it through independently learning agents. 

In contrast, we introduce a Status-Quo ($SQLoss$) that evolves cooperation between agents without sharing rewards, gradients, or using a communication channel.  The $SQLoss$ encourages an agent to imagine the consequences of sticking to the status-quo. This imagined stickiness ensures that an agent gets a better estimate of a cooperative or selfish policy. Without $SQLoss$, agents repeatedly switch policies (from cooperative to selfish), obtain short-term rewards (through exploitation), and, therefore incorrectly learn that a selfish strategy gives higher rewards in the long-term.
%Figure~\ref{fig:results_IPD} shows how $SQLoss$ compares to existing approaches to evolve cooperative behavior in multi-agent reinforcement learning games.

% To work with social dilemma games that have visual observations, we introduce \ipdistill. \ipdistill uses self-supervision and clustering to automatically extract a cooperative and a selfish policy from a social dilemma game. The input to \ipdistill is a collection of state sequences derived from random game-play between two random agents. Each state sequence represents a collection of states and actions (of both agents), leading up to a reward in the environment. \ipdistill uses this collection of state sequences to learn two oracles. One oracle represents a cooperative policy, and the other oracle represents a selfish policy. Given a state, an oracle returns an action according to the specific policy. 
\changed{The approach using $SQLoss$ has been designed for single-step or normal form games that are repeatedly played. This can be extended to multi-step (extensive form) games by using teh standard extensive form to normal form conversion from game theory [REF]. However, this converted normal form game has actions equal to the number of strategies in the original multi-step game, which may be practically intractable. Hence, we propose an approach that reduces this normal form game by clustering the new action space, i.e., the policy space of the original multi-step game. This approach can be summarized as follows. We first encode the trajectories (sequences of states and actions of all agents) of game play into features that are sufficient to predict the outcomes. These features are then clustered and corresponding oracles (inferred policies) are extracted from these clusters. In sequential social dilemmas, since policies can be grouped into either cooperation or defection policies, we cluster features into two distinct clusters and extract the corresponding cooperation and defection oracles. We then apply $SQLoss$ to this reduced game using these extracted policies as actions of the reduced equivalent normal form game.}
It is important to note that each agent independently runs \ipdistill to extract oracles. For instance, Figure~\ref{fig:oracle_predictions} (Appendix~\ref{appendix:oracle:illustration}) illustrates the cooperation and defection oracles extracted by the Red agent using \ipdistill in the Coin Game.
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/high_level_approach_new_horizontal.pdf}
    \caption{High-level architecture of our approach. Each agent runs \ipdistill by performing $(1), (2), (3)$ individually before playing the social dilemma game. This creates two oracles per agent. During game-play$(4)$, each agent (enhanced with $SQLoss$) takes either the action suggested by the cooperation oracle or the action suggested by the defection oracle.}
    \label{fig:high_level_approach}
\end{figure*}
% \begin{enumerate}
%     \item For a social dilemma game with visual observations, each RL agent runs \ipdistill to learn oracles that implement cooperative and selfish behavior. 
%     \item We train agents (with $SQLoss$) to play the game such that at any step, an agent can either take the action suggested by the cooperation oracle or the selfish oracle. 
% \end{enumerate}
% We empirically demonstrate in Section~\ref{sec:results} that our approach evolves cooperative behavior between independently trained agents.

% In this paper, we present a novel MARL algorithm that allows independently learning Deep RL agents to converge to \textbf{individually and socially desirable cooperative behavior} in such social dilemma situations. 

Our key contributions in this paper can be summarised as:
\begin{enumerate}
    \item We introduce a \textbf{Status-Quo} loss ($SQLoss$, Section~\ref{sec:approach:SQLoss}) and an associated policy gradient-based algorithm that learns optimal behavior in sequential social dilemma iterated matrix games that conforms to human behavior in such games (Section \ref{sec:results}). 
    % We empirically demonstrate that agents trained with the $SQLoss$ evolve optimal behavior in several social dilemma iterated matrix games (Section \ref{sec:results}).
    \item We propose \ipdistill (Section~\ref{sec:GameDistill}), an algorithm that reduces a multi-step social dilemma game to an iterated matrix game by extracting policies that implement cooperative and selfish behavior. We empirically demonstrate that \ipdistill extracts cooperative and selfish policies for the Coin Game (Section~\ref{sec:results:visual-input-gamedistll-and-sqloss}). 
    \item We demonstrate that when agents run \ipdistill followed by MARL game-play using $SQLoss$, they converge to individually as well as socially desirable cooperative behavior in single and multi-step sequential social dilemmas. (Section~\ref{sec:results:visual-input-gamedistll-and-sqloss}).
\end{enumerate}

\begin{comment}
This result is particularly interesting because behavioral economists~\cite{samuelson1988status, kahneman1991anomalies, kahneman2011thinking, thaler2009nudge} have studied the effect of the Status-Quo bias in decision making in humans. Our work shows that it is possible that the Status-Quo bias helps to evolve cooperative behavior in human groups. They start with two policies, cooperation (denoted by $\pi_C$) and defection (denoted by $\pi_D$). They use these policies to generate intermediate policies with varying degrees of Cooperation and Defection. During game-play, each agent predicts the degree of cooperation of its opponent and chooses a policy of the same degree of cooperation. We propose an IPD-Distilling architecture (\ipdistill) to transform a multi-agent game to its IPD formulation. \ipdistill uses self-supervision and clustering to learn cooperation and defection policies automatically. We use \ipdistill to transform a game to an IPD, followed by $SQLoss$ enhanced agents to evolve cooperative behavior for RL agents in the Coin game \cite{foerster2018learning}. We show that RL agents trained using our approach achieve higher levels of cooperation and average reward than those trained with existing approaches (Section~\ref{sec:results}).
%Figure~\ref{fig:high_level_approach} shows a high-level description of our approach. 

\end{comment}



\begin{comment}

\citet{consequentialist18} take the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and have built in a handcrafted mechanism of playing multiple roll-outs of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule based mechanism to choose between cooperation($\pi_C$) and defection ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 
\end{comment}



==> main-content/approach_only_sqloss.tex <==
\section{Approach}
\label{sec:approach}
%\begin{figure*}
%    \includegraphics[width=\linewidth]{images/skill_detection_network.png}
%    \caption{Network architecture diagram for skill discovery network}
%    \label{fig:skill_detection_network}
%\end{figure*}
%\begin{figure}
%    \includegraphics[width=\linewidth]{images/action_prediction_network.png}
%    \caption{Neural Network architecture for the Action Prediction Network}
%    \label{fig:action_prediction_network}
%\end{figure}
%Figure~\ref{fig:high_level_approach} shows the high-level architecture of our approach.

\subsection{Social Dilemmas modeled as Iterated Matrix Games}
To remain consistent with previous work, we adopt the notations from \citet{foerster2018learning}.
We model social dilemmas as general-sum Markov (simultaneous move) games. A multi-agent Markov game is specified by $G = \langle$$S$, $A$, $U$, $P$, $r$, $n$, $\gamma$$\rangle$. $S$ denotes the state space of the game. $n$ denotes the number of agents playing the game.
At each step of the game, each agent $a \in A$, selects an action $u^a \in U$. $\Vec{u}$ denotes the joint action vector that represents the simultaneous actions of all agents. The joint action $\Vec{u}$ changes the state of the game from $s$ to $s'$ according to the state transition function $P(s'|\Vec{u},s): S \times \textbf{U} \times S \rightarrow  [0, 1]$. At the end of each step, each agent $a$ gets a reward according to the reward function $r^{a}(s, \Vec{u}): S \times \textbf{U} \rightarrow \mathbb{R}$. The reward obtained by an agent at each step is a function of the actions played by all agents. For an agent $a$, the discounted future return from time $t$ is defined as $R_{t}^{a} = \sum_{l=0}^{\infty} \gamma^{l} r_{t+l}^{a}$, where $\gamma \in [0, 1)$ is the discount factor. Each agent independently attempts to maximize its expected discounted return. 

Matrix games are the special case of two-player perfectly observable Markov games~\cite{foerster2018learning}.  Table~\ref{tab:payoff_matrix} shows examples of matrix games that represent social dilemmas. 
Consider the Prisoner's Dilemma game in Table~\ref{tab:payoff_matrix_ipd}. Each agent can either cooperate (\textit{C}) or defect (\textit{D}). Playing \textit{D} is the logical choice for an agent, regardless of whether the other agent plays \textit{C} or \textit{D}. Therefore, if both agents play logically, each receives a reward of $-2$. 
However, if each agent plays \textit{C}, then it will obtain a reward of $-1$. This fact that individually rational behavior leads to a poor group (and individual) outcomes highlights the dilemma. 

In Infinitely Iterated Matrix Games, agents repeatedly play a particular matrix game against each other. 
In each iteration of the game, each agent has access to actions played by both agents in the previous iteration. Therefore, the state input to an RL agent consists of both agents' actions in the previous iteration of the game.
We use only the actions played in the previous iteration since ??? show that ???
% We adopt this state formulation as is typically done in such games \cite{press2012iterated, foerster2018learning}.
% The infinitely iterated variations of the matrix games in Table~\ref{tab:payoff_matrix} represent sequential social dilemmas. 
We refer to infinitely iterated matrix games as iterated matrix games in subsequent sections for convenience. 

\subsection{Learning Policies in Social Dilemmas: The Selfish Learner}
\label{sec:approach:selfish-learner}
A straightforward method to model agents in iterated matrix games is to model each agent as an RL agent that independently attempts to maximize its expected total discounted reward. Several approaches to model agents in this way use policy gradient-based methods~\cite{sutton2000policy, williams1992simple}. Policy gradient methods update an agent's policy, parameterized by $\theta^{a}$, by performing gradient ascent on the expected total discounted reward $\E [R_{0}^{a}]$. Formally, let $\theta^{a}$ denote the parameterized version of an agent's policy $\pi^{a}$ and $V_{\theta^{1},\theta^{2}}^{a}$ denote the total expected discounted reward for agent $a$.  Here, $V^{a}$ is a function of the policy parameters $(\theta^{1}, \theta^{2})$ of both agents. In the $i^{th}$ iteration of the game, each agent updates $\theta_{i}^{a}$ to $\theta_{i+1}^{a}$, such that it maximizes it's total expected discounted reward. $\theta_{i+1}^{a}$ is computed using Eq.~\ref{eq:theta_argmax}. For agents trained using reinforcement learning, the gradient ascent rule to update $\theta_{i+1}^{1}$ is given by Eq.~\ref{eq:naive_learner_update_rule}.
\begin{equation}
    % \small
    % \begin{split}
        \theta_{i+1}^{1} = \argmax_{\theta^{1}} V^{1}(\theta^{1}, \theta_{i}^{2}) %\\
        ~~~\text{and}~~~
        \theta_{i+1}^{2} = \argmax_{\theta^{2}} V^{2}(\theta_{i}^{1}, \theta^{2})
    \label{eq:theta_argmax}%
    % \end{split}
\end{equation}%
\begin{equation}%
    % \begin{split}
        f_{nl}^{1} = \nabla_{\theta^{i}_{1}} V^{1} (\theta_{i}^{1}, \theta_{i}^{2}) \cdot \delta ~~~\text{and}~~~
        \theta_{i+1}^{1} = \theta_{i}^{1} + f_{nl}^{1} (\theta_{i}^{1}, \theta_{i}^{2}) 
    % \end{split}
    \label{eq:naive_learner_update_rule}%
\end{equation}
where $\delta$ is the step size of the updates.


In the Iterated Prisoner's Dilemma (IPD), agents trained with the policy gradient update method converge to a mutual defection equilibrium (Figure~\ref{fig:results_IPD}, \citet{Peysakhovich1707.01068}). 
This poor reward outcome attained by Selfish Learners motivates us to explore alternative methods that could lead to a higher reward equilibrium. 
We denote the agent trained using policy gradient updates as a Selfish Learner ($SL$).

\subsection{Learning Policies in Social Dilemmas: The Status-Quo Aware Learner ($SQLoss$)}
\label{sec:approach:SQLoss}
%Figure~\ref{fig:high_level_approach} shows the high-level architecture of our approach.
\subsubsection{$SQLoss$: Motivation and Theory}
\label{sec:approach:SQLoss:intuition}
%The status-quo bias instills in humans a preference for the current state provided the state is not harmful to them. 
Inspired by the human behavioral idea of a preference for the status-quo, we introduce a status-quo loss ($SQLoss$) for RL, derived from the idea of imaginary game-play (Figure~\ref{fig:rl_imaginative_learning}). 
\begin{figure}[hbt!]
    \centering
    \includegraphics[width=0.55\linewidth]{images/rl_gameplay_summary_new_horizontal__sqlearner_only.pdf}
    \caption{Intuition behind \textit{Status-Quo}-aware learner. At each step, the $SQLoss$ encourages an agent to imagine the consequences of sticking to the status-quo by imagining an episode where the status-quo is repeated for $\kappa$ steps.
    For instance, in $S_{1}$, an agent receives $r_{0}$ and imagines an episode where it remains in $S_{1}$ for $\kappa$ steps, receiving $r_{0}$ at each step.
    Section~\ref{sec:approach:SQLoss} describes $SQLoss$ in more detail.
    }
    \label{fig:rl_imaginative_learning}
\end{figure}

This idea of imagining a $\kappa$-step continuation of the status-quo makes agents more likely to punish defection and reward cooperation, thereby encouraging long-term mutual cooperation.
% $SQLoss$ encourages an agent to imagine a future episode where the status-quo (current situation) is repeated for several steps. 
If an agent has been exploited in the previous iteration of the game (state \textit{DC}), then $SQLoss$ will encourage the agent to imagine a continued risk of exploitation and subsequently switch to defection and move to state \textit{DD}.  
Hence, for the exploiting agent, the short-term gain from exploitation (\textit{DC}) is overcome by the long-term loss from mutual defection (\textit{DD}). 
Conversely, if both agents cooperated in the previous iteration of the game (state \textit{CC}), then $SQLoss$ will encourage the agent to imagine a continued gain from mutual cooperation and subsequently stick to state \textit{CC}.
Since state \textit{CC} is more beneficial to both agents than \textit{DD}, and exploitation (\textit{DC} and \textit{CD}) also leads to \textit{DD}, agents move away from defection and converge to mutual cooperation (\textit{CC}). 
Section~\ref{section:emergence-of-cooperation} describes in more detail how cooperation emerges between $SQLoss$ agents.
% Therefore, agents move towards mutual cooperation $(CC)$ or mutual defection $(DD)$. With exploitation (and subsequently, the fear of being exploited) being discouraged, agents move towards cooperation.
% Why do independent, selfish learners converge to mutually harmful behavior in the IPD? To understand this, consider the payoff matrix for a single iteration of the IPD in Table~\ref{tab:payoff_matrix_ipd}. In each iteration, an agent can play either \textit{C} or \textit{D}. Mutual defection $(DD)$ is worse for each agent than mutual cooperation $(CC)$. However, one-sided exploitation (\textit{DC} or \textit{CD}) is better than mutual cooperation for the exploiter and far worse for the exploited. Therefore, as long as an agent perceives the possibility of exploitation, it is drawn to defect, both to maximize the reward (through exploitation) and minimize its loss (through being exploited). To increase the likelihood of cooperation, it is important to reduce instances of exploitation between agents. 
% We posit that, if agents either mutually cooperate $(CC)$ or mutually defect $(DD)$, then they will learn to prefer \textit{C} over \textit{D} and achieve a socially desirable equilibrium.  (for a detailed illustration of the evolution of cooperation, see Appendix~\ref{appendix:sqloss_theory}, which is part of the Supplementary Material)  

% Motivated by ideas from human psychology that attribute cooperation in humans to the status-quo bias~\cite{guney2018costly}, we introduce a status-quo loss ($SQLoss$) for each agent, derived from the idea of imaginary game-play (Figure~\ref{fig:rl_imaginative_learning}). 
% Intuitively, the loss encourages an agent to imagine an episode where the status-quo (current situation) is repeated for several steps. This imagined episode causes the exploited agent (in \textit{DC}) to perceive a continued risk of exploitation and, therefore, quickly move to $(DD)$. 
% Hence, for the exploiting agent, the short-term gain from exploitation $(DC)$ is overcome by the long-term loss from mutual defection $(DD)$. 
% Therefore, agents move towards mutual cooperation $(CC)$ or mutual defection $(DD)$. With exploitation (and subsequently, the fear of being exploited) being discouraged, agents move towards cooperation.


\subsubsection{$SQLoss$: Formulation}
\label{sec:approach:SQLoss:formulation}
We describe below the formulation of SQLoss with respect to agent 1. The formulation for agent 2 is identical to that of agent 1. Let $\uptau_a = (s_{0}, u_{0}^{1}, u_{0}^{2}, r_{0}^{1}, \cdots s_{T}, u_{T}^{1}, u_{T}^{2}, r_{T}^{1})$ denote the collection of an agent's experiences after $T$ time steps. Let $R_{t}^{1} (\uptau_1) = \sum_{l=t}^{T} \gamma^{l-t} r_{l}^{1}$ denote the discounted future return for agent $1$ starting at $s_t$ in actual game-play. Let $\hat \uptau_{1}$ denote the collection of an agent's \textbf{imagined} experiences. For a state $s_{t}$, where $t \in [0, T]$, an agent imagines an episode by starting at $s_{t}$ and repeating $u_{t-1}^{1}, u_{t-1}^{2}$ for $\kappa_{t}$ steps. This is equivalent to imagining a $\kappa_{t}$ step repetition of already played actions. We sample $\kappa_{t}$ from a Discrete Uniform distribution $\mathbb{U} \{1,z\}$ where $z$ is a hyper-parameter $\geq 1$. To simplify notation, let $\phi_t(s_t, \kappa_{t})$ denote the ordered set of state, actions, and rewards starting at time $t$ and repeated $\kappa_{t}$ times for imagined game-play. Let $\hat R_{t}^{1} (\hat \uptau_1)$ denote the discounted future return starting at $s_t$ in imagined status-quo game-play.
{
    % \setlength{\abovedisplayskip}{-3pt}
    % \setlength{\belowdisplayskip}{-4pt}
    \begin{equation}%
        \small
        \phi_t(s_t,\kappa_{t}) = \big[ (s_{t}, u_{t-1}^{1}, u_{t-1}^{2}, r_{t-1}^{1})_0,
        ~\cdots (s_{t}, u_{t-1}^{1}, u_{t-1}^{2}, r_{t-1}^{1})_1, (s_{t}, u_{t-1}^{1}, u_{t-1}^{2}, r_{t-1}^{1})_{\kappa_{t}-1} \big]
    \end{equation}%
}%
{%
    % \setlength{\abovedisplayskip}{1pt}
    % \setlength{\belowdisplayskip}{-2pt}
    \begin{equation}%
        \small
        \hat \uptau_{1} = \big( \phi_t(s_t,\kappa_{t}), (s_{t+1}, u_{t+1}^{1}, u_{t+1}^{2}, r_{t+1}^{1})_{\kappa_{t} + 1}, ~\cdots~, (s_{T}, u_{T}^{1}, u_{T}^{2}, r_{T}^{1})_{T+\kappa_{t}-t} \big)
        % \label{eq:tau_hat}
    \end{equation}%
}%
\begin{equation}%
    \small
    % R_{t}^{1} (\uptau_1) & = \sum_{l=t}^{T} \gamma^{l-t} r_{l}^{1} \\
    \hat R_{t}^{1} (\hat \uptau_1) = \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) r_{t-1}^{1} + \gamma^{\kappa} R_{t}^{1} (\uptau_1) = \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) r_{t-1}^{1} + \gamma^{\kappa} \sum_{l=t}^{T} \gamma^{l-t} r_{l}^{1}
    \label{eq:returns_hat}
\end{equation}%
$V_{\theta^{1},\theta^{2}}^{1}$ and $\hat V_{\theta^{1},\theta^{2}}^{1}$ are approximated by $\E [R_{0}^{1} (\uptau_1)]$ and $\E[\hat R_{0}^{1} (\hat \uptau_1)]$ respectively. These $V$ values are the expected rewards conditioned on both agents' policies ($\pi^{1}$, $\pi^{2}$). For agent 1, the regular gradients and the Status-Quo gradient-like correction term, $\nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)]$ and $f_{sqcor}^{1}$, can be derived from the policy gradient formulation as
% \begin{equation}
%     \small
%     \begin{split}
%         \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] = \E  [R_{0}^{1}(\uptau_1)\nabla_{\theta^{1}} \log\pi^{1}(\uptau_1)]
%         & = \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}}  \log\pi^{1} (u_{t}^{1}|s_{t}) \cdot \sum_{l=t}^{T} \gamma^{l} r_{l}^{1} {\Big]} \\
%         & = \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}}  \log\pi^{1} (u_{t}^{1}|s_{t}) \gamma^{t} \big( R_{t}^{1}(\uptau_1) - b(s_{t}) \big) \Big]
%     \end{split}
%     \label{eq:pg_original}
% \end{equation}%
\begin{equation}
    \small
    \begin{split}
        \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] = \E  [R_{0}^{1}(\uptau_1)\nabla_{\theta^{1}} \log\pi^{1}(\uptau_1)]
        % & = \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}}  \log\pi^{1} (u_{t}^{1}|s_{t}) \cdot \sum_{l=t}^{T} \gamma^{l} r_{l}^{1} {\Big]} \\
        & = \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}}  \log\pi^{1} (u_{t}^{1}|s_{t}) \gamma^{t} \big( R_{t}^{1}(\uptau_1) - b(s_{t}) \big) \Big]
    \end{split}
    \label{eq:pg_original}
\end{equation}%
\vspace{-7pt}
% \begin{equation}%
%     \small
%     \begin{split}%
%         \nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\hat \uptau_1)] & = \E~[\hat R_{0}^{1}(\hat \uptau_1)\nabla_{\theta^{1}} \log\pi^{1}(\hat \uptau_1)] \\
% % \cdot
%         & = \E {\Bigg[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \times
%         \Bigg( \sum_{l=t}^{t+\kappa} \gamma^{l} r_{t-1}^{1} + \sum_{l=t}^{T} \gamma^{l+\kappa} r_{l}^{1} \Bigg) \Bigg]\\
% %
%         & = \E {\Bigg[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \times
%         \Bigg( \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) \gamma^{t} r_{t-1}^{1} + \gamma^{\kappa} \sum_{l=t}^{T} \gamma^{l} r_{l}^{1} \Bigg) \Bigg] \\
% %
%         &= \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \gamma^{t} \big( \hat R_{t}^{1}(\hat \uptau_1) - b(s_{t}) \big) \Big]
%     \end{split}
%     \label{eq:status_quo_pg}
% \end{equation}
\begin{equation}%
    \small
    \begin{split}%
        % \nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\hat \uptau_1)] & = \E~[\hat R_{0}^{1}(\hat \uptau_1)\nabla_{\theta^{1}} \log\pi^{1}(\hat \uptau_1)] \\
        f_{sqcor}^{1}
% \cdot
        % & = \E {\Bigg[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \times
        % \Bigg( \sum_{l=t}^{t+\kappa} \gamma^{l} r_{t-1}^{1} + \sum_{l=t}^{T} \gamma^{l+\kappa} r_{l}^{1} \Bigg) \Bigg]\\
%
        & = \E {\Bigg[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \times
        \gamma^{t} \times \Bigg( \Big( \frac{1 - \gamma^{\kappa}}{1 - \gamma} \Big) r_{t-1}^{1} + \gamma^{\kappa} \sum_{l=t}^{T} \gamma^{l - t} r_{l}^{1} - b(s_{t}) \Bigg) \Bigg] \\
%
        &= \E {\Big[} \sum_{t=1}^{T} \nabla_{\theta^{1}} \log\pi^{1} (u_{t-1}^{1}|s_{t}) \times \gamma^{t} \times \big( \hat R_{t}^{1}(\hat \uptau_1) - b(s_{t}) \big) \Big]
    \end{split}
    \label{eq:status_quo_pg}
\end{equation}
Here, $f_{sqcor}^{1}$ in Eq.~\ref{eq:status_quo_pg} is a biased term that has policy gradient-like structure and incorporates the prior action taken through the $u_{t-1}|s_t$ term.
It should be noted that the $f_{sqcor}^{1}$ is not a gradient of the expected return of the imagined trajectory in Eq.~\ref{eq:returns_hat}, but the form of this expression is arrived at considering the policy gradient expression. 
Furthermore, $b(s_t)$ is a baseline-like term added for variance reduction in the implementation. 
% The key idea behind $SQLoss$ is the $u_{t-1}|s_t$ term. This term causes the agent to focus on the action taken to arrive at the current state, rather than the action taken in the current state ($u_{t}|s_t$). Simply summing/repeating rewards or lowering the discount factor would still operate on the ($u_{t}|s_t$) term and therefore not achieve a similar effect.

The update rule $f_{sql,pg}$ for the policy gradient-based Status-Quo Learner (SQL-PG) is defined by,
% \begin{equation}
%     % \small
%     f_{sql,pg}^{1} = \big( \alpha \cdot \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] + \beta \cdot \nabla_{\theta^{1}} \E [\hat R_{0}^{1}(\uptau_1)] \big) \cdot \delta
% \end{equation}
\begin{equation}
    % \small
    f_{sql,pg}^{1} = \big( \alpha \cdot \nabla_{\theta^{1}} \E [R_{0}^{1}(\uptau_1)] + \beta \cdot f_{sqcor}^{1} \big) \cdot \delta
\end{equation}
where $\alpha$, $\beta$ are the loss scaling factor for REINFORCE and imaginative game-play respectively.
\begin{table}
    \centering
    \small
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \small
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{c|c|c}
             & \textit{C} & \textit{D} \\ \hline
             \textit{C} & (-1, -1) & (-3, 0) \\ \hline
             \textit{D} & (0, -3) & (-2, -2) \\ \hline
        \end{tabular}
        \caption{Prisoners' Dilemma (PD)}
        \label{tab:payoff_matrix_ipd}
    \end{subtable}%
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \small
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{c|c|c}
             & \textit{H} & \textit{T} \\ \hline
             \textit{H} & (+1, -1) & (-1, +1) \\ \hline
             \textit{T} & (-1, +1) & (+1, -1) \\ \hline
        \end{tabular}
        \caption{Matching Pennies (MP)}
        \label{tab:payoff_matrix_imp}
    \end{subtable}%
    \begin{subtable}[t]{0.3\linewidth}
        \centering
        \small
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{c|c|c}
             & \textit{C} & \textit{D} \\ \hline
             \textit{C} & (0, 0) & (-4, -1) \\ \hline
            %  \textit{C} & (4, 4) & (0, 3) \\ \hline
             \textit{D} & (-1, -4) & (-3, -3) \\ \hline
            %  \textit{D} & (3, 0) & (1, 1) \\ \hline
        \end{tabular}
        \caption{Stag Hunt (SH)}
        \label{tab:payoff_matrix_sh}
    \end{subtable}%
    \caption{\label{tab:payoff_matrix}%
    Payoff matrices for the different games used in our experiments. $(X,Y)$ in a cell represents a reward of $X$ to the row and $Y$ to the column player. \textit{C}, \textit{D}, \textit{H}, and \textit{T} denote the actions for the row and column players. In the iterated versions of these games, agents play against each other over several iterations. In each iteration, an agent takes an action and receives a reward based on the actions of both agents. Each matrix represents a different kind of social dilemma.}%
    \vspace{-13pt}
\end{table}%

\subsubsection{$SQLoss$: Emergence of Cooperation}
\label{section:emergence-of-cooperation}
Equation~\ref{eq:pg_original} (Section~\ref{sec:approach:SQLoss:formulation}) describes the gradient for standard policy gradient. 
It has two terms.
The $log\pi^{1} (u_{t}^{1}|s_{t})$ term maximises the likelihood of reproducing the training trajectories $[(s_{t-1},u_{t-1},r_{t-1}),(s_{t},u_{t},r_{t}),(s_{t+1},u_{t+1},r_{t+1}),\dots]$.
The return term pulls down trajectories that have poor return.
The overall effect is to learn a policy that can reproduce high-return trajectories.
We refer to this standard loss as $Loss$ for the following discussion.
\begin{lemma}
    \label{section:lemma:lemma1}
    For agents trained with random exploration in the IPD, $Q_{\pi}(D|s_t) > Q_{\pi}(C|s_t)$ for all $s_t$.
\end{lemma}
Let $Q_{\pi}(a_t|s_t)$ denote the expected return of taking $a_t$ in $s_t$.
Let $V_{\pi}(s_t)$ denote the expected return from state $s_t$.
\begin{equation}
    \begin{split}
        Q_{\pi}(C|CC) &= 0.5*\big((-1) \; + \; V_{\pi}(CC)\big) \; + \; 0.5*\big((-3) + V_{\pi}(CD)\big)\\
        Q_{\pi}(C|CC) &= -2 \; + \; 0.5*\big(V_{\pi}(CC) + V_{\pi}(CD)\big)\\
        Q_{\pi}(D|CC) &= -1 \; + \; 0.5*\big(V_{\pi}(DC) + V_{\pi}(DD)\big)\\
        Q_{\pi}(C|CD) &= -2 \; + \; 0.5*\big(V_{\pi}(CC) + V_{\pi}(CD)\big)\\
        Q_{\pi}(D|CD) &= -1 \; + \; 0.5*\big(V_{\pi}(DC) + V_{\pi}(DD)\big)\\
        Q_{\pi}(C|DC) &= -2 \; + \; 0.5*\big(V_{\pi}(CC) + V_{\pi}(CD)\big)\\
        Q_{\pi}(D|DC) &= -1 \; + \; 0.5*\big(V_{\pi}(DC) + V_{\pi}(DD)\big)\\
        Q_{\pi}(C|DD) &= -2 \; + \; 0.5*\big(V_{\pi}(CC) + V_{\pi}(CD)\big)\\
        Q_{\pi}(D|DD) &= -1 \; + \; 0.5*\big(V_{\pi}(DC) + V_{\pi}(DD)\big)
    \end{split}
\end{equation}
Since $V_{\pi}(CC)=V_{\pi}(CD)=V_{\pi}(DC)=V_{\pi}(DD)$ for randomly playing agents, $Q_{\pi}(D|s_t) > Q_{\pi}(C|s_t)$ for all $s_t$.

\begin{lemma}
\label{lemma:lemma2}
Agents trained to only maximize the expected reward in IPD will converge to mutual defection. 
\end{lemma}
This lemma follows from Lemma~\ref{section:lemma:lemma1}.
Agents initially collect trajectories from random exploration. 
They use these trajectories to learn a policy that optimizes for long-term return. 
These learned policies always play $D$ as described in Lemma~\ref{section:lemma:lemma1}.

Equation 7 describes the gradient for $SQLoss$. 
The $log\pi^{1} (u_{t-1}^{1}|s_{t})$ term maximises the likelihood of taking $u_{t-1}$ in $s_{t}$.
The imagined episode return term pulls down trajectories that have poor imagined return. 

\begin{lemma}
\label{lemma:lemma3}
Agents trained on random trajectories using only $SQLoss$ oscillate between $CC$ and $DD$. 
\end{lemma}

For the game, $s_{t} = (u_{t-1}^{1}, u_{t-1}^{2})$.
The $SQLoss$ maximises the likelihood of taking $u_{t-1}$ in $s_{t}$ when the return of the imagined trajectory $\hat R_{t}(\hat \uptau_1)$ is high.


Consider state $CC$, with $u_{t-1}^{1}=C$.
$\pi^{1} (D|CC)$ is randomly initialised. 
The $SQLoss$ term reduces the likelihood of $\pi^{1} (C|CC)$ because $\hat R_{t}(\hat \uptau_1) < 0$. 
Therefore, $\pi^{1} (D|CC) > \pi^{1} (C|CC)$.

Similarly, for $CD$, the $SQLoss$ term reduces the likelihood of $\pi^{1} (C|CD)$.
Therefore, $\pi^{1} (D|CD) > \pi^{1} (C|CD)$.
For $DC$, $\hat R_{t}(\hat \uptau_1) = 0$, therefore $\pi^{1} (D|DC) > \pi^{1} (C|DC)$.
Interestingly, for $DD$, the $SQLoss$ term reduces the likelihood of $\pi^{1} (D|DD)$ and therefore $\pi^{1} (C|DD) > \pi^{1} (D|DD)$. 

Now, if $s_t$ is $CC$ or $DD$, then $s_{t+1}$ is $DD$ or $CC$ and these states oscillate. 
If $s_t$ is $CD$ or $DC$, then $s_{t+1}$ is $DD$, $s_{t+2}$ is $CC$ and again $CC$ and $DD$ oscillate. 
This $CC$, $DD$ oscillation is key to the emergence of cooperation.

\begin{lemma}
\label{lemma:lemma4}
For agents trained using both standard loss and $SQLoss$, $\pi (C|CC) > \pi^{1} (D|CC)$.
\end{lemma}
For $CD$, $DC$, both the standard loss and $SQLoss$ push the policy towards $D$.
For $DD$, with sufficiently high $\kappa$, the $SQLoss$ term overcomes the standard loss and pushes the agent towards $C$.
For $CC$, initially, both the standard loss and $SQLoss$ push the policy towards $D$.
However, as training progresses, the incidence of $CD$ and $DC$ diminish because of $SQLoss$ as described in Lemma 3.
Therefore, $V_{\pi}(CD) \approx V_{\pi}(DC)$ since agents immediately move from both states to $DD$. 
Intuitively, agents lose the opportunity to exploit the other agent. 
In equation 9, with $V_{\pi}(CD) \approx V_{\pi}(DC)$, $Q_{\pi}(C|CC) > Q_{\pi}(D|CC)$ and the standard loss pushes the policy so that $\pi (C|CC) > \pi (D|CC)$. 
This depends on the value of $\kappa$.
For very low values, the standard loss overcomes $SQLoss$ and agents defect.
For very high values, $SQLoss$ overcomes standard loss, and agents oscillate between cooperation and defection.
For moderate values of $\kappa$ (as shown in our experiments), the two loss terms work together so that $\pi (C|CC) > \pi (D|CC)$.


\subsection{Learning Policies in Visual Input Social Dilemmas using $SQLoss$}
\label{section:visual-input-games}
$SQLoss$ requires that the action space contains two actions (typically a cooperation and a defection action) and is therefore not directly applicable to visual input games (such as the Coin Game, Appendix~\ref{appendix:game-details}) where cooperation and defection policies are composed of a sequence of lower level actions (such as up, down, left, right).
To apply the Status-Quo policy gradient to these games, we train cooperation and defection oracles by training agents using the sum-of-rewards for both agents and individual reward, respectively~\cite{Peysakhovich1707.01068}.
During game-play, an agent can consult either oracle at each step. 
In the Coin Game, this is equivalent to either cooperating (consulting the cooperation oracle) or defecting (consulting the defection oracle). 
In this way, an agent reduces the game to its matrix equivalent. 
We then utilize the Status-Quo policy gradient to learn policies in the reduced matrix game.
For the Coin Game, this leads to agents who cooperate by only picking coins of their color (Figure~\ref{fig:coingame_results}).

%The previous section focused on learning optimal policies in iterated matrix games that represent sequential social dilemmas. 
%In such games, an agent can take one of a discrete set of policies at each step. 
%For instance, in IPD, an agent can either cooperate or defect at each step. 
%However, in social dilemmas such as the Coin Game (Appendix~\ref{appendix:game-details}), cooperation and defection policies are composed of a sequence of state-dependent actions.


\begin{comment}
For any game, the idea is summarized as follows:
\begin{enumerate}
    \item \textbf{N complex actions -> M complex skills:} Learning decoupled skills has multiple benefits as they can be easily transferred to other agents, or new skills can be learned, or skills can be updated.  This also decouples the environment-specific information from the skills of the agents.
    \item \textbf{Action Prediction Network:} Once the skills are identified, this module converts the meta-learning (in the form of skill) to environment-specific actions/interactions. This allows the agents to behave a certain way in the environment given a skill.
    \item \textbf{Skill selection policy:} Given agents can interact with the environment given a skill/policy, now the task boils down to selecting a skill at a given state that maximizes the overall reward of the agents.
\end{enumerate}
\end{comment}


\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{images/meta_policy.png}
    \caption{Reduction of a game to an IPD formulation. We summarize complex skills using oracles and the agent has to learn a meta-policy to switch between skills. \todopb{Make a formal version of this reduction}}
    \label{fig:meta_policy}
\end{figure}
\end{comment}


==> main-content/checklist.tex <==
\section{Reproducibility Checklist}
We follow the reproducibility checklist from \href{https://www.cs.mcgill.ca/~jpineau/ReproducibilityChecklist.pdf~}~\cite{reproducibility_checklist} and include further details here. For all the models and algorithms we have included details that we think would be useful for reproducing the results of this work.
\begin{itemize}a
\item For all \textbf{models} and \textbf{algorithms} presented, check if you include:
\begin{enumerate}
    \item \textit{A clear description of the mathematical setting, algorithm, and/or model}: \textbf{Yes}. The algorithm is described in detail in Section~\ref{sec:approach}, with all the loss functions used for training being clearly defined. The details of the architecture, hyperparameters used and other algorithm details are given in Section~\ref{sec:experimental_setup}. Environment details are explained in the sections that they are introduced in.
    \item \textit{A clear explanation of any assumptions.}: \textbf{Yes}. We provide all the assumptions that we have made in the model design or the experiments wherever required.
    \item \textit{An analysis of the complexity (time, space, sample size) of any algorithm}: \textbf{No}. We do not include a formal complexity analysis of our algorithm. However, we do highlight the additional computational steps (in terms of losses and parameter updates) in Section~\ref{sec:approach} over standard multi-agent independently learning RL algorithms that would be needed in our approach.
    \item \textit{A link to a downloadable source code, with specification of all dependencies, including external libraries.}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
\end{enumerate}
 
 
 
\item For any \textbf{theoretical claim}, check if you include:
\begin{enumerate}
    \item \textit{A statement of the result}: \textbf{NA}. Our paper is primarily empirical and we do not have any major theoretical claims. Hence this is Not Applicable.
    \item \textit{A clear explanation of any assumptions}: \textbf{NA}.  
    \item \textit{A complete proof of the claim}: \textbf{NA}.
\end{enumerate}
 
\item For all \textbf{figures} and \textbf{tables} that present empirical results, check if you include:
\begin{enumerate}
    \item \textit{A complete description of the data collection process, including sample size}: \textbf{NA}. We did not collect any data for our work.
    \item \textit{A link to a downloadable version of the dataset or simulation environment}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
    \item \textit{An explanation of any data that were excluded, description of any pre-processing step}: \textbf{NA}. We did not perform any pre-processing step.
    \item \textit{An explanation of how samples were allocated for training / validation / testing}: \textbf{Yes}. For \ipdistill the details regarding data used for training is given in Section~\ref{sec:GameDistill}. The number of iterations used for learning (training) by $SQLearner$ is given in Figures~\ref{fig:results_IPD},~\ref{fig:results_IMP} and~\ref{fig:coingame_results}. The details of the number of runs and the batch sizes used for various experiments are given in Section~\ref{sec:experimental_setup}.
\end{enumerate}

\item For all \textbf{reported experimental results}, check if you include:
\begin{enumerate}
    \item \textit{The range of hyper-parameters considered, method to select the best hyper-parameter configuration, and specification of all hyper-parameters used to generate results}: \textbf{Yes}. We did not perform any hyper-parameter tuning as part of this work. All the hyper-parameters that we used are specified in Section~\ref{sec:experimental_setup}.
    \item \textit{The exact number of evaluation runs}: \textbf{Yes}. For all our environments, we repeat the experiment $20$ times. For evaluation of performance, we use an average of $200$ Monte Carlo estimates. We state this in Section~\ref{sec:experimental_setup}. We do not need to fix any seed. In order to test reproducibility use the seed in the code. The details of the number of runs and the batch sizes used for various experiments are also provided.
    \item \textit{A description of how experiments were run}: \textbf{Yes}. The README with instructions on how to run the experiments along with the source code is provided at~\citet{github_code}.
    \item \textit{A clear definition of the specific measure or statistics used to report results}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{Clearly defined error bars}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{A description of results with central tendency (e.g. mean) \& variation (e.g. stddev)}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
    \item \textit{The average runtime for each result, or estimated energy cost}: \textbf{Yes}. We have provided this detail in the README along with the code. It takes approximately 25 minutes to finish around 60 training epochs which should be enough time to get the results. It is also a hard stop based on the parameters above. If the code execution ends prematurely then consider increasing the --num-episodes parameter to get the results.
    \item \textit{A description of the computing infrastructure used}: \textbf{Yes}. We have provided this detail in the Supplementary material in Appendix~\ref{appendix:experimental-setup:computation-req}.
\end{enumerate}
\end{itemize}

==> main-content/checklist_neuroips.tex <==
\section*{Checklist}

% \section{Reproducibility Checklist}
% We follow the reproducibility checklist from \href{https://www.cs.mcgill.ca/~jpineau/ReproducibilityChecklist.pdf~}~\cite{reproducibility_checklist} and include further details here. For all the models and algorithms we have included details that we think would be useful for reproducing the results of this work.
% \begin{itemize}a
% \item For all \textbf{models} and \textbf{algorithms} presented, check if you include:
% \begin{enumerate}
%     \item \textit{A clear description of the mathematical setting, algorithm, and/or model}: \textbf{Yes}. The algorithm is described in detail in Section~\ref{sec:approach}, with all the loss functions used for training being clearly defined. The details of the architecture, hyperparameters used and other algorithm details are given in Section~\ref{sec:experimental_setup}. Environment details are explained in the sections that they are introduced in.
%     \item \textit{A clear explanation of any assumptions.}: \textbf{Yes}. We provide all the assumptions that we have made in the model design or the experiments wherever required.
%     \item \textit{An analysis of the complexity (time, space, sample size) of any algorithm}: \textbf{No}. We do not include a formal complexity analysis of our algorithm. However, we do highlight the additional computational steps (in terms of losses and parameter updates) in Section~\ref{sec:approach} over standard multi-agent independently learning RL algorithms that would be needed in our approach.
%     \item \textit{A link to a downloadable source code, with specification of all dependencies, including external libraries.}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
% \end{enumerate}
 
 
 
% \item For any \textbf{theoretical claim}, check if you include:
% \begin{enumerate}
%     \item \textit{A statement of the result}: \textbf{NA}. Our paper is primarily empirical and we do not have any major theoretical claims. Hence this is Not Applicable.
%     \item \textit{A clear explanation of any assumptions}: \textbf{NA}.  
%     \item \textit{A complete proof of the claim}: \textbf{NA}.
% \end{enumerate}
 
% \item For all \textbf{figures} and \textbf{tables} that present empirical results, check if you include:
% \begin{enumerate}
%     \item \textit{A complete description of the data collection process, including sample size}: \textbf{NA}. We did not collect any data for our work.
%     \item \textit{A link to a downloadable version of the dataset or simulation environment}: \textbf{Yes}. We have made the source code available at \citet{github_code}.
%     \item \textit{An explanation of any data that were excluded, description of any pre-processing step}: \textbf{NA}. We did not perform any pre-processing step.
%     \item \textit{An explanation of how samples were allocated for training / validation / testing}: \textbf{Yes}. For \ipdistill the details regarding data used for training is given in Section~\ref{sec:GameDistill}. The number of iterations used for learning (training) by $SQLearner$ is given in Figures~\ref{fig:results_IPD},~\ref{fig:results_IMP} and~\ref{fig:coingame_results}. The details of the number of runs and the batch sizes used for various experiments are given in Section~\ref{sec:experimental_setup}.
% \end{enumerate}

% \item For all \textbf{reported experimental results}, check if you include:
% \begin{enumerate}
%     \item \textit{The range of hyper-parameters considered, method to select the best hyper-parameter configuration, and specification of all hyper-parameters used to generate results}: \textbf{Yes}. We did not perform any hyper-parameter tuning as part of this work. All the hyper-parameters that we used are specified in Section~\ref{sec:experimental_setup}.
%     \item \textit{The exact number of evaluation runs}: \textbf{Yes}. For all our environments, we repeat the experiment $20$ times. For evaluation of performance, we use an average of $200$ Monte Carlo estimates. We state this in Section~\ref{sec:experimental_setup}. We do not need to fix any seed. In order to test reproducibility use the seed in the code. The details of the number of runs and the batch sizes used for various experiments are also provided.
%     \item \textit{A description of how experiments were run}: \textbf{Yes}. The README with instructions on how to run the experiments along with the source code is provided at~\citet{github_code}.
%     \item \textit{A clear definition of the specific measure or statistics used to report results}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
%     \item \textit{Clearly defined error bars}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
%     \item \textit{A description of results with central tendency (e.g. mean) \& variation (e.g. stddev)}: \textbf{Yes}. We plot the mean and the one standard deviation region over the mean for all our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.
%     \item \textit{The average runtime for each result, or estimated energy cost}: \textbf{Yes}. We have provided this detail in the README along with the code. It takes approximately 25 minutes to finish around 60 training epochs which should be enough time to get the results. It is also a hard stop based on the parameters above. If the code execution ends prematurely then consider increasing the --num-episodes parameter to get the results.
%     \item \textit{A description of the computing infrastructure used}: \textbf{Yes}. We have provided this detail in the Supplementary material in Appendix~\ref{appendix:experimental-setup:computation-req}.
% \end{enumerate}
% \end{itemize}




%%% BEGIN INSTRUCTIONS %%%
% \answerYes{}
% \answerNo{}
% \answerNA{}

%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Our paper is primarily empirical and we do not have any major theoretical claims. For all the other claims we provide multiple empirical studies in Sections~\ref{sec:experimental_setup} and ~\ref{sec:results}.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations of our work in Section~\ref{sec:GameDistill}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We don't foresee any negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have followed the guidelines as mentioned in the above documents.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Our paper is primarily empirical and we do not have any major theoretical claims. We have minor supporting theoretical statements in the Supplementary material. For all the other claims we provide multiple empirical studies in Sections~\ref{sec:experimental_setup} and ~\ref{sec:results}}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{Though the paper does not have any theoretical claims, we have provided proofs for the minor theoretical supporting statements in the Supplementary Material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We have made the source code available at \citet{github_code} and provided the instructions along with the source code.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We have provided details our of experimental setup in Section~\ref{sec:experimental_setup}. We have also provided extensive details of our experimental settings in Section~\ref{appendix:experimental-setup} in the Supplementary Material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We plot the mean and the one standard deviation region (exceptions to this are stated in the figure caption) over the mean for our numerical experiments. This is stated in Section~\ref{sec:experimental_setup}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We have provided details of the type of resources used in Section~\ref{appendix:experimental-setup:computation-req} in the Supplementary Material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{We have included the license along with the code.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide the additional assets along with the source code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We have not used the data obtained from the people.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> main-content/experimental_setup_only_sqloss.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}
In order to compare our results to previous work, we use the Normalized Discounted Reward $NDR = (1-\gamma) \sum_{t=0}^{T} \gamma^{t} r_{t}$. 
A higher NDR implies that an agent obtains a higher reward in the environment. 
We compare our approach (Status-Quo Aware Learner or $SQLearner$) to Learning with Opponent-Learning Awareness (Lola-PG)~\cite{foerster2018learning} and the Selfish Learner (SL) agents.
For all experiments, we perform $20$ runs and report average $NDR$, along with variance across runs. 
The bold line in all the figures is the mean, and the shaded region is the one standard deviation region around the mean.
All of our code is available at \href{https://github.com/user12423/MARL-with-SQLoss/}{Github-MARL-with-SQLoss}

\subsection{Social Dilemmas Modeled as Iterated Matrix Games}
For our experiments with social dilemmas, we use the Iterated Prisoners Dilemma (IPD)~\cite{luce1989games}, Iterated Matching Pennies (IMP)~\cite{lee1967application}, and the Iterated Stag Hunt (ISH)~\cite{fang2002adaptive}. 
% We show results on stag hunt as it describes a conflict between safety and social cooperation and presents an example of ``trust dilemma'' between players. 
% The stag hunt differs from the Prisoner's Dilemma in that there are two pure-strategy Nash equilibria when both players cooperate and both players defect. 
% In contrast, in the Prisoner's Dilemma, the only pure Nash equilibrium is when both players defect, despite the fact that both players cooperating is Pareto efficient. 
Each matrix game in Table~\ref{tab:payoff_matrix} represents a different dilemma.  
% In the Prisoner's Dilemma, the logical policy for each agent is to defect, regardless of the other agent's policy.
% However, when each agent plays rationally, each is worse off. 
In Matching Pennies, if an agent plays predictably, it is prone to exploitation by the other agent. 
Therefore, the optimal policy is to randomize between \textit{H} and \textit{T}, obtaining an average NDR of $0$. 
The Stag Hunt game represents a coordination dilemma. 
In the game, given that the other agent will cooperate, an agent's optimal action is to cooperate as well. 
However, each agent has an attractive alternative at each step, that of defecting and obtaining a guaranteed reward of $-1$. 
Therefore, the promise of a safer alternative and the fear that the other agent might select the safer choice could drive an agent to select the safer alternative, thereby sacrificing the higher reward of mutual coordination. 

In iterated matrix games, for each iteration (iter), agents take an action according to a policy and receive the rewards in Table~\ref{tab:payoff_matrix}. 
To simulate an infinitely iterated game, we let agents play 200 iters of the matrix game against each other, and do not provide an agent with any information about the number of remaining iters. 
In an iter, the state for an agent is the actions played by both agents in the previous iter.

Further, LOLA transforms the game matrix to contain non-positive values as a preprocessing step.
To remain consistent with LOLA, we have performed the same preprocessing on all games.
For a general matrix game, we can subtract the maximum reward (or any number larger than it) from each reward value to make rewards negative and then use $SQLoss$. 
% Further, $SQLoss$ works on a version of the game in which all rewards have been transformed to non-positive values. 
% For the matrix games described in our paper, we have used their variants with negative rewards to remain consistent with LOLA.

\begin{comment}
We consider the social dilemma class of matrix games from \citet{Leibo:2017},
\begin{equation}
    \small
    \begin{pmatrix}
        & C & D \\ 
        C & R,R & S,T \\
        D & T,S & P,P \\
    \end{pmatrix}
\end{equation}%
where the first row corresponds to cooperation for the first player and the first column corresponds to cooperation for the second player. 
\citet{Leibo:2017} define the following rules that describe different categories of social dilemmas: 
\textbf{(i)} If $R > P$, then mutual cooperation is preferred to mutual defection. 
\textbf{(ii)} If $R > S$, then mutual cooperation is preferred to being exploited by a defector. 
\textbf{(iii)} If $2R > T + S$, this ensures that mutual cooperation is preferred to an equal probability of unilateral cooperation and defection.
\textbf{(iv)} Either greed ($T > R$: Exploit a cooperator preferred over mutual cooperation) or fear ($P > S$: Mutual defection preferred over being exploited) should hold.
% \begin{enumerate}
%     \item If $R > P$, then mutual cooperation is preferred to mutual defection.
%     \item If $R > S$, then mutual cooperation is preferred to being exploited by a defector.
%     \item If $2R > T + S$, this ensures that mutual cooperation is preferred to an equal probability of unilateral cooperation and defection.
%     \item Either greed ($T > R$: Exploit a cooperator preferred over mutual cooperation) or fear ($P > S$: Mutual defection preferred over being exploited) should hold.
% \end{enumerate}%
These rules have been reproduced from \citet{Leibo:2017},%
\begin{enumerate}%
    \item When ``greed'' ($T > R$) as well as ``fear'' ($P > S$) conditions hold, we have $T > R > P > S$. The Iterated Prisoner's Dilemma (IPD) is an example of this game. If we subtract $T$ from each reward, we get the matrix game.
    \begin{equation}%
        \small
        \begin{pmatrix}
            & C & D \\
            C & R-T,R-T & S-T,0 \\
            D & 0,S & P-T,P-T \\
        \end{pmatrix}
    \end{equation}%
    where all entries are non-positive and therefore Lemma 3 and Lemma 4 hold as before.
    \item When ``greed'' holds but not ``fear'' we have $T > R > S >= P$. The Chicken Game (CG) is an example of this game. If we subtract $T$ from each reward as before, we get the equivalent matrix game with non-positive entries and Lemmas 3 and 4 hold.
    \item When ``fear'' holds but not ``greed'' we have $R >= T > P > S$. The Iterated Stag Hunt is an example of this game. If we subtract $R$ from each reward, we get the equivalent matrix game with non-positive entries then Lemmas~\ref{lemma:lemma3} and~\ref{lemma:lemma4} (Appendix~\ref{appendix:sqloss_theory}) hold.
\end{enumerate}
In our experiments, we have considered games from each of the classes mentioned above, and the use of $SQLoss$ leads to cooperation in all these examples.
\end{comment}

\subsection{Social Dilemmas Modeled as Visual Input Games}
\label{section:approach:social-dilemmas-as-visual-input-games}
For our experiments on social dilemmas with visual input and extended actions, we use the Coin Game (Figure~\ref{fig:coin_game})~\cite{foerster2018learning} and the visual input variant of the Stag Hunt (Figure~\ref{fig:stag_hunt_game}). 
We provide details of the games in Appendix~\ref{appendix:game-details} due to space considerations.
% For the Coin Game, the rational policy for an agent is to defect and try to pick all coins, regardless of the policy of the other agent. However, when both agents defect, both are worse off.

==> main-content/introduction_only_sqloss.tex <==
\section{Introduction}
\label{sec:introduction}
\begin{comment}
\begin{figure}[ht]
    \includegraphics[width=\linewidth]{images/overall_idea.png}
    \caption{A schematic diagram of the proposed idea}
    \label{fig:overall_idea}
\end{figure}
\end{comment}
% In intertemporal social dilemmas, there is a tradeoff between short-term individual incentives and long-term collective interest. Humans face such dilemmas when contributing to collective food storage during the summer in preparation for a harsh winter, organizing annual maintenance of irrigation systems, or sustainably sharing a local fishery. Classical models of human behavior based on rational choice theory predict that cooperation in these situations is impossible [1, 2]. This poses a puzzle since humans evidently do find ways to cooperate in many everyday intertemporal social dilemmas, as documented by decades of fieldwork [3, 4] and laboratory experiments [5, 6]. Providing an empirically grounded explanation of how individual behavior gives rise to societal cooperation is seen as a core goal in several subfields of the social sciences and evolutionary biology [7, 8, 9].[10, 11] proposed influential models based on behavioral game theory. However, these models have limited applicability since they only generate predictions when the problem can be cast as a matrix game (see e.g. [12, 13]). Here we consider a more realistic video-game setting, like those introduced in the behavioral research of [14, 15, 16]. In this environment, agents do not simply choose to cooperate or defect like they do in matrix games. Rather they must learn policies to implement their strategic decisions and must do so while coping with the non-stationarity arising from other agents learning simultaneously. Several papers used multi-agent reinforcement learning [17, 18, 19] and planning [20, 21, 22, 23] to generate cooperation in this setting. However, this approach has not yet demonstrated robust cooperation in games with more than two players, which is often observed in human behavioral experiments. Moreover naïvely optimizing group reward is also ineffective, due to the lazy agent problem [24].
%It is difficult for both natural and artificial agents to find cooperative solutions to intertemporal social dilemmas for the following reasons:
%1. Collective action – individuals must learn and coordinate policies at a group level to avoid falling into socially deficient equilibria.
%2. Temporal credit assignment – rational defection in the short-term must become associated with long-term negative consequences.
%Many different research traditions, including economics, evolutionary biology, sociology, psychology, and political philosophy have all converged on the idea that fairness norms are involved in resolving social dilemmas [25, 26, 27, 28, 29, 30, 31]. In one well-known model, agents are assumed to have inequity-averse preferences [10]. They balance their selfish desire for individual rewards against a need to keep deviations between their own rewards and the rewards of others as small as possible. Inequity-averse individuals are able to solve social dilemmas by resisting the temptation to pull ahead of others or—if punishment is possible—by punishing and discouraging free-riding. The inequity aversion model has been successfully applied to explain human behavior in a variety of laboratory economic games, such as the ultimatum game, the dictator game, the gift exchange game, market games, the trust game, and public goods

%Google paper
% Social dilemmas expose tensions between collective and individual rationality [1]. Cooperation makes possible better outcomes for all than any could obtain on their own. However, the lure of free riding and other such parasitic strategies implies a tragedy of the commons that thickens the stability of any cooperative venture [2]. 
%The theory of picked general-sum matrix games provides a framework for understanding social dilemmas. Fig. 1 shows payoff matrices for three canonical examples: Prisoner's Dilemma, Chicken, and Stag Hunt. The two actions are interpreted as cooperating and defect respectively. The four possible outcomes of each stage game are R (a reward of mutual cooperation), P (punishment arising from mutual defection), S (sucker outcome obtained by the player who cooperates with a defecting partner), and T (temptation outcome achieved by defecting against a cooperator).
%A matrix game is a social dilemma when its four payoffs satisfy the following social dilemma inequalities (this formulation from [3]):
%1. R > P Mutual cooperation is preferred to mutual defection. (1)
%2. R > S Mutual cooperation is preferred to being exploited by a defector. (2)
%3. 2R > T +S This ensures that mutual cooperation is preferred to an equal probability of unilateral cooperation and defection. (3)
%4. either greed: T > R Exploiting a cooperator is preferred over mutual cooperation or fear: P > S Mutual defection is preferred over being exploited. (4)
%Matrix Game Social Dilemmas (MGSD) have been fruitfully employed as models for a wide variety of phenomena in theoretical social science and biology.


% \textcolor{red}{http://www.ifaamas.org/Proceedings/aamas2019/pdfs/p1877.pdf}


In sequential social dilemmas, individually rational behavior can lead to outcomes that are sub-optimal for each individual in the group \citet{Hardin1968,ostrom:1990,Ostrom278,Dietz1907}. 
Current state-of-the-art Multi-Agent Deep Reinforcement Learning (MARL) methods that train agents independently lead to agents that play individualistically and receive lower rewards, even in simple social dilemmas \cite{foerster2018learning, Peysakhovich1707.01068}.
%(Section~\ref{sec:approach:selfish-learner}). % cooperate reliably This failure to cooperate results in sub-optimal individual and group outcomes

Such dilemmas represent a conflict where a collection of individually rational policies lead to outcomes that are poor for the group of individuals. 
Consider the Coin Game (first explored in ~\cite{foerster2018learning}).
Each agent can play either selfishly (pick all coins) or cooperatively (pick only coins of its color). 
Regardless of the other agent's behavior, the individually rational choice for an agent is to play selfishly, either to minimize losses (avoid being exploited) or to maximize gains (exploit the other agent).
However, when both agents behave rationally, they try to pick all coins and achieve an average long term reward of $-0.5$. 
In contrast, if both play cooperatively, then the average long term reward for each agent is $0.5$. 
Therefore, when agents cooperate, they are both better off. \abhishek{Too deep an explanation of the game, can shorten it }
Training Deep RL agents independently in the Coin Game using state-of-the-art methods leads to mutually harmful selfish behavior (Section~\ref{sec:approach:selfish-learner}).

Interestingly, humans develop individual and socially beneficial strategies in such social dilemmas without sharing rewards or having access to private information. 
Several ideas in human psychology~\cite{samuelson1988status, kahneman1991anomalies, kahneman2011thinking, thaler2009nudge} have attributed this cooperative behavior to the status-quo bias~\cite{guney2018costly}.
The status-quo bias is a decision-making bias that encourages humans to stick to the status-quo unless doing so causes significant harm. 
This preference in humans for sticking to `comfortable' states rather than seeking short-term exploitative gains is one explanation for emergent cooperative behavior in human groups.


Inspired by this idea, we present the status-quo loss ($SQLoss$) and the corresponding status-quo policy gradient formulation for RL.  
% Intuitively, $SQLoss$ encourages an agent to repeat past behaviour unless such repetition causes significant harm. 
Agents trained with $SQLoss$ achieve high returns in multi-agent social dilemmas without sharing rewards, gradients, or using a communication channel.
% Intuitively, $SQLoss$ encourages an agent to stick to the action taken previously, with the encouragement proportional to the reward received previously. 
% The introduction and motivation for SQLoss needs improvement. The "status quo bias" is the central concept in the paper. Hence, in the introduction, the authors must define it precisely (rather than simply relying on references, or even worse, relying on people's 'common sense' understanding of the term). The authors also should explain the main reason from human psychology that it leads to cooperation in social dilemmas. Currently, the text merely states the term and immediately explains their proposed SQLoss, saying that "SQLoss encourages an agent to stick to the action taken previously". I doubt "status-quo bias" exactly means "stick to the action taken previously". More importantly, the authors themselves say in Section 2.3.1 that "this imagined episode causes the exploited agent in (DC) to perceive a continued risk of exploitation and, therefore, quickly move to (DD)". Hence it is not correct to say that "SQLoss encourages an agent to stick to the action taken previously".
Intuitively, $SQLoss$ encourages an agent to stick to past actions provided these actions did not cause significant harm.
Therefore, mutually cooperating agents stick to cooperation since the status-quo yields higher individual reward, while unilateral defection by any agent leads to the other agent also switching to defection since the status-quo is harmful for the exploited agent. 
Subsequently, for each agent, the short-term reward of exploitation is overcome by the long-term cost of mutual defection, and agents gradually switch to cooperation (Section \ref{sec:approach:SQLoss}). 
% imagine the consequences of sticking to the status quo. 
% Imagining this counterfactual at every step helps agents derive more accurate estimates of a cooperation or defection policy. 
% Without $SQLoss$, agents repeatedly switch policies (from cooperation to defection), obtain short-term rewards (through exploitation), and, therefore incorrectly learn that a defection strategy gives higher rewards in the long-term.
%Figure~\ref{fig:results_IPD} shows how $SQLoss$ compares to existing approaches to evolve cooperative behavior in multi-agent reinforcement learning games.

% To apply $SQLoss$ to games where a sequence of non-trivial actions determines cooperation and defection, we present \ipdistill, an algorithm that reduces a dynamic game with visual input to a matrix game. 
% To work with social dilemma games that have visual observations, we introduce \ipdistill. 
% In the Coin Game, each agent uses \ipdistill independently to extract cooperation and a defection policy.  
% independently to obtain two oracles representing a cooperative and a selfish policy where each oracle returns an action according to the specific policy. 
% We empirically demonstrate in Section~\ref{sec:results} that agents trained with $SQLoss$ on a \ipdistill reduced version of the Coin Game evolve optimal policies. 


% In this paper, we present a novel MARL algorithm that allows independently learning Deep RL agents to converge to \textbf{individually and socially desirable cooperative behavior} in such social dilemma situations.
Our key contributions can be summarised as:
\begin{enumerate}[topsep=0pt,itemsep=1ex,partopsep=1ex,parsep=1ex]
    \item We introduce a \textbf{Status-Quo} loss ($SQLoss$, Sec.~\ref{sec:approach:SQLoss}) and an associated policy gradient-based algorithm to learn optimal behavior in a decentralized manner for agents playing iterated games where agents can choose between a cooperative and selfish policy at each iteration. 
    We empirically demonstrate that agents trained with $SQLoss$ achieve high rewards in several social dilemma matrix games (Sec. \ref{sec:results}).
    \item We extend $SQLoss$ to social dilemma games with visual observations by reducing these games to their matrix equivalent using pre-trained cooperation and defection oracles (Section \ref{section:visual-input-games}). 
    \item We demonstrate that $SQLoss$ extends in a straight forward manner to games with more than two agents due to its ego-centric nature (Sec.~\ref{sec:beyond_2_players}).
\end{enumerate}
% \section{Related Work}
The problem of how independently learning agents learn behavior in social dilemmas has been studied by researchers through human studies and simulation models~\cite{Fudenberg, Edward:1984, Fudenberg:1984, Kamada:2010, Abreu:1990}. 
A large body of work has looked at the mechanism of evolution of cooperation through reciprocal behaviour and indirect reciprocity~\cite{reciprocal1971,reciprocal1984,reciprocal1992,reciprocal1993,in_reciprocal1998}, through variants of reinforcement using aspiration~\cite{reinforce_variant}, attitude~\cite{NonRL_attitude} or multi-agent reinforcement learning~\cite{Sandholm1996MultiagentRL,Wunder:2010}, and under specific conditions~\cite{R_plus_S_g_2P} using different learning rates \cite{deCote:2006} similar to WoLF~\cite{WOLF2002} as well as using embedded emotion~\cite{Emotional_Multiagent}, social networks~\cite{Ohtsuki2006,Santos:2006}.
\abhishek{This looks like a paragraph to go in the related works? Not really needed here. Also can change the citation style to display numbers instead of author names. Can just mention a few of the related works here, and remaining in the related work section?}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/high_level_approach_new_horizontal.pdf}
    \caption{High-level architecture illustrated using coin game. Each agent runs \ipdistill by performing steps $(1), (2), (3)$ individually to obtain two oracles per agent. During game-play$(4)$, each agent (with $SQLoss$) takes either the action suggested by the cooperation or the defection oracle}
    \label{fig:high_level_approach}
\end{figure*}

However, these approaches do not directly apply to Deep RL agents~\cite{Leibo:2017}. 
Recent work in this direction~\cite{kleiman2016coordinate,Julien:2017,consequentialist18} focuses on letting agents learn strategies through interactions with other agents in a multi-agent setting. 
\citet{Leibo:2017} defines the problem of social dilemmas in the Deep RL framework and analyzes the outcomes of a fruit-gathering game~\cite{Julien:2017}. 
% They vary the abundance of resources and the cost of conflict in the fruit environment to generate degrees of cooperation between agents. 
\citet{Hughes:2018} defines an intrinsic reward (inequality aversion) that attempts to reduce the difference in obtained rewards between agents. 
% The agents are designed to have an aversion to both advantageous (guilt) and disadvantageous (unfairness) reward allocation. 
% This handcrafting of loss with mutual fairness develops cooperation, but it leaves the agent vulnerable to exploitation. 
LOLA~\cite{foerster2018learning} uses opponent awareness to achieve high cooperation levels in the Coin Game and the Iterated Prisoner's Dilemma game. 
The LOLA agent assumes access to the other agent's network architecture, observations, and learning algorithms.  
% This access level is analogous to getting complete access to the other agent's private information and therefore devising a strategy with full knowledge of how they are going to play.  
\citet{Wang:2019} proposes an evolutionary Deep RL setup to learn cooperation. 
They define an intrinsic reward that is based on features generated from the agent's past and future rewards, and this reward is shared with other agents. 
They use evolution to maximize the sum of rewards among the agents and thus learn cooperative behavior. 
% Sharing rewards in this indirect way enforces cooperation rather than evolving it through independently learning agents. 
% add line saying we are building on these approaches .... 


$SQLoss$ is different from these methods since agents trained with $SQLoss$ achieve high returns in multi-agent settings without sharing rewards~\cite{Wang:2019}, gradients~\cite{foerster2018learning}, handcrafting reward functions~\cite{Julien:2017}, using a communication channel, or modeling the other agent(s)~\cite{foerster2018learning}.
% Hysteresis and leniency are alternate methods explored in the literature~\cite{WeiL16,Palmer:2019}.
\abhishek{Again this paragraph is just literature review. No need to mention all approaches, and even if you are mentioning it should be max 1 line for each. I think only LOLA can be mentioned here}


\begin{comment}
This result is particularly interesting because behavioral economists~\cite{samuelson1988status, kahneman1991anomalies, kahneman2011thinking, thaler2009nudge} have studied the effect of the Status-Quo bias in decision making in humans. Our work shows that it is possible that the Status-Quo bias helps in evolving cooperative behavior in human groups. They start with two policies, cooperation (denoted by $\pi_C$) and defection (denoted by $\pi_D$). They use these policies to generate intermediate policies with varying degrees of Cooperation and Defection. During game-play, each agent predicts the degree of cooperation of its opponent and chooses a policy of the same degree of cooperation. We propose an IPD-Distilling architecture (\ipdistill) to transform a multi-agent game to its IPD formulation. \ipdistill uses self-supervision and clustering to learn cooperation and defection policies automatically. We use \ipdistill to transform a game to an IPD, followed by $SQLoss$ enhanced agents to learn cooperative behavior for RL agents in the Coin game \cite{foerster2018learning}. We show that RL agents trained using our approach achieve higher levels of cooperation and average reward than those trained with existing approaches (Section~\ref{sec:results}).
%Figure~\ref{fig:high_level_approach} shows a high-level description of our approach. 
\end{comment}



\begin{comment}
\citet{consequentialist18} takes the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and has built-in a handcrafted mechanism of playing multiple roll-outs of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule-based mechanism to choose between cooperation($\pi_C$) and defection ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 
\end{comment}



==> main-content/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Social dilemma problems brings out the conflict between an individual and the society and
Prisoner's dilemma \cite{Rapoport1974} has been used to highlight this core conflict. In-spite of several examples of cooperation in nature at various scales, from microscopic \cite{Szathmary1995}, to species level \cite{Heinsohn1995ComplexCS} including humans\cite{kleiman2016coordinate}, still greedy behavior leads to tragedy of the commons \cite{psychology_social_dilemmas}

There has been a large body of work which had looked at the mechanism of emergence of cooperation through reciprocal behaviour and indirect reciprocity \cite{reciprocal1971},\cite{reciprocal1984},\cite{reciprocal1992},\cite{reciprocal1993},\cite{in_reciprocal1998}, though variants of reinforcement using aspiration \cite{reinforce_variant}, attitude\cite{NonRL_attitude} or using multi-agent reinforcement learning \cite{Sandholm1996MultiagentRL,Wunder:2010}, under specific conditions \cite{R_plus_S_g_2P}, using different learning rates \cite{deCote:2006} similar to WoLF \cite{WOLF2002} as well as using embedded emotion \cite{Emotional_Multiagent}.

But with the advent of deep reinforcement learning~\cite{Mnih:2013,Mnih:2015}, recent work on social dilemma problem have taken a rather hands off approach with the idea of letting agents figure out strategies, all by themselves. In the paper~\cite{Leibo:2017} the authors have setup the problem of social dilemma in deep reinforcement learning framework and have analyzed the outcome of the 2d Fruit gathering game as general sum matrix games, where by varying the abundance of resources and cost of conflict, they generate varying degrees of cooperation. In~\cite{Hughes:2018}, they define an intrinsic reward called inequality aversion which tries to reduce difference in rewards among the agents by having aversion to both advantageous(guilt) and disadvantageous(unfairness) inequity. This handcrafting of loss with mutual fairness leads to better cooperation but also makes the agent vulnerable to exploitation. The authors in~\cite{foerster2018learning} propose LOLA, where they achieve high degree of cooperation in their Coin game and Iterative Prisoner's Dilemma. They do this by having access to the opponent policy parameters and gradients. This is equivalent to getting access to opponent's brain and devising strategy with the knowledge of how they are about to play. In a more recent paper~\cite{Wang:2019}, \citeauthor{Wang:2019} proposes an evolutionary based deep reinforcement learning setup to evolve cooperation. They define an intrinsic reward which is based on a feature, generated from agent's past and expected future rewards and this feature is shared with other agents. They then use evolution to maximise the sum of rewards among the agents which leads to achieving cooperation. This is an indirect method of maximizing the sum of rewards for the society which would lead to cooperation.
Another paper \cite{Wang:2018} proposed a method, where they start with two policies, cooperation($\pi_C$) and defection ($\pi_D$). With these they generate several intermediate policies with varying degrees of ($\pi_C$) and ($\pi_D$) and then during gameplay each agent tries to predict the degree of cooperation by its opponent and chooses a matching policy of same degree of cooperation. This is an indirect way of hard coding a strategy like Tit-For-Tat because both agent try to mimic the opponent's perceived policy rather than playing to maximize their respective rewards. In contrast to these methods we try to develop cooperation using a status-quo loss, without inducing any strategy bias towards cooperation.

In \cite{consequentialist18}, \citeauthor{consequentialist18} takes the direction of having predefined policies of cooperation($\pi_C$) and defection ($\pi_D$) and have built in a handcrafted mechanism of playing multiple rollouts of actions $CC$ and $CD$ to figure out the payoffs for these strategies. Subsequently, they use a rule based mechanism to choose between cooperation($\pi_C$) and defection ($\pi_D$) policies. Their idea of having existing policies of ($\pi_C$) and ($\pi_D$) is similar to our idea of learning skills of cooperation or defection. However, we try to discover these policies using a self-supervised clustering method while playing the game in a random manner (i.e. random action policy). 

% \citet{kleiman2016coordinate} studied the emergence of cooperation and defection for humans and compare it results from agents learnt using reinforcement-learning.

==> main-content/results_only_sqloss.tex <==
\section{Results}
\label{sec:results}
% \label{sec:results}
% \begin{figure*}[!th]
%     \centering
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{3d-feature-vec.png}
%         \caption{3-dimensional feature vector}
%         \label{fig:clustering_3d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/4d-feature-vec.png}
%         \caption{4-dimensional feature vector}
%         \label{fig:clustering_4d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/10d-feature-vec.png}
%         \caption{10-dimensional feature vector}
%         \label{fig:clustering_10d}
%     \end{subfigure}\hfil%
%     \begin{subfigure}[t]{.5\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{images/100d-feature-vec.png}
%         \caption{100-dimensional feature vector}
%         \label{fig:clustering_100d}
%     \end{subfigure}%
% \caption{\label{fig:feature_vector_plots}%
% In each subfigure, Left figures represent the actual rewards obtained by both the agents (the ground-truth), while the figures on the Right represent the clusters obtained by Agglomerative Clustering (when no-of-clusters was set to 2). For feature vectors of higher dimensions (>2), we show their t-SNE~\cite{maaten2008visualizing} projections. In the figures on the left, the Legend shows the events that give $Agent_{1}$ a reward of $r_{1}$ and $Agent_{2}$ a reward of $r_{2}$ denoted in the format \textbf{$r_{1}$|$r_{2}$}. In the plots on the right, from the legend, Class $0$ and Class $1$ represent the Cooperation and Defection clusters respectively. From the figures, all the events that resulted in the opponent getting penalized belong to the same cluster, namely the Defection cluster.}
% \end{figure*}

\begin{comment}

\subsection{Learning optimal policies in Iterated Matrix Games through an $\eta$-stationary environment}
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{images/ipd_results_sticky=5.png}
        \caption{($\eta=5$)-Stationary environment}
        \label{fig:ipd_results_sticky=5}
    \end{subfigure}\hfil%
    \begin{subfigure}[t]{0.4\linewidth}
        \includegraphics[width=\linewidth]{images/ipd_results_sticky=20.png}
        \caption{($\eta=20$)-Stationary environment}
        \label{fig:ipd_results_sticky=20}
    \end{subfigure}%
    \caption{Instantaneous probability of cooperation for two selfish learner agents in the IPD game when the environment enforces stationarity. The Green line indicates the probability of cooperation and the Blue line the probability of defection. When the level of stationarity enforced by the environment is high (20), even selfish learners develop cooperation.}
    \label{fig:ipd_results_with_sticky}%
\end{figure*}
%\begin{figure}[h]
%    \includegraphics[width=0.4\textwidth]{images/ipd_results_action_loss_at_t=1_and_t=2_sticky=10.png}
%    \caption{Instantaneous probability of cooperation for both the agents in the IPD game when the environment enforces the sticky policy with stickiness=20 and the agents are penalized only at t=2 step of the sticky game-play for action-loss.}
%    \label{fig:ipd_results_action_loss_at_t=1_and_t=2_sticky=10}
%\end{figure}
% \begin{figure}[h]
%     \includegraphics[width=0.4\textwidth]{images/ipd_results_with_futuristic_state_loss.png}
%     \caption{Average Probability of cooperation for both the agents in a traditional IPD game with the proposed imaginative-learning loss.}
%     \label{fig:ipd_results_with_futuristic_state_loss}
% \end{figure}
%\begin{figure}[h]
%    \includegraphics[width=0.4\textwidth]{images/ipd_results_with_futuristic_state_loss__variance_K=1-2.png}
%    \caption{Average Probability of cooperation for both the agents in a traditional IPD game with the proposed imaginative-learning loss with $\kappa$ varying from 1 to 2 (both inclusive).  \textcolor{green}{Green} line indicates probability of cooperation while \textcolor{blue}{Blue} line indicates probability of defection}
%    \label{fig:ipd_results_with_futuristic_state_loss__with_variance}
%\end{figure}


\paragraph{\textbf{Iterated Prisoner's Dilemma (IPD):}}
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{images/results__IPD__nash_eq_almost.png}
    \caption{Average NDR values for different learners in the IPD game. The reward graph for $a0$ is hidden because of the overlap with the graph for $a1$. $SQLearner$ agents obtain a near-optimal NDR value (-1) for this game.}
    \label{fig:results_IPD}
\end{figure}
To validate our hypothesis that Selfish Learners learn cooperative behavior in a stationary environment, we train two $SL$ agents in the IPD game using a $5$-stationary environment and a $20$-stationary environment. Figure \ref{fig:results_IPD} shows the results. As expected, we see that enforcing stationarity in the environment induces cooperative behavior between independently trained agents. In the $20$-stationary environment, the probability of agents cooperating is close to 1 (agents always cooperate).  We also observe that the probability of cooperation sharply drops every few epochs. We believe that these sudden drops are due to the inherent incentive to exploit the other agent. However, once the agents realize that mutual exploitation is harmful, they revert to cooperative behavior. The interval between consecutive drops in cooperation probability reduces as training proceeds.

We obtain similar results for a $10$-stationary environment; however, in this case, it took longer for the agents to converge to cooperation. We have omitted the figure for space considerations. Interestingly, in the $5$-stationary environment (Figure~\ref{fig:ipd_results_sticky=5}), agents do not converge to cooperation. This result implies a minimum environment stationarity threshold required for agents to overcome short-term exploitation considerations and converge to cooperation. For IPD, we find that this stationarity threshold is equal to ... 


%Developing motivation from the \textit{sticky policy} results, we further experiment with breaking-down stickiness to understand its impact on the learning of the agents. In a traditional IPD game, agents are penalized at each decision. However, with a sticky policy enforced in the environment, the environment ideally only requests for the action once every sticky game-play. However, penalizing only at every sticki'th step would convert it into a traditional game. We then experiment with propagating loss only at t=2 step of the sticky game-play. Fig~\ref{fig:ipd_results_action_loss_at_t=1_and_t=2_sticky=10} shows that the agents learn to cooperate with loss at just t=2 step of the sticky game-play for the action loss. Interestingly, having a mask at the action-value loss is enough to assist agents in learning to cooperate.

Figure~\ref{fig:imp_results_with_sticky} and Figure~\ref{fig:ish_results_with_sticky} in Appendix A show the probability of cooperation for $SL$ agents trained in the \textbf{IMP} and \textbf{ISH} game respectively. For both games, we find that agents develop optimal policies when the environment is stationary.
\end{comment}

\subsection{Iterated Matrix Games}
\label{sec:results:iterated-matrix-games:sqloss}

\textbf{Iterated Prisoner's Dilemma (IPD):}
% \begin{figure}[htb!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/IPD_results_corrected.png}
%     \caption{\label{fig:results_IPD}%
%     Average NDR values for different learners in the IPD game. 
%     $SQLearner$ agents obtain a near-optimal NDR value $(-1)$ for this game. 
%     In contrast to other methods, $SQLearner$ agents have close to zero variance across runs. 
%     }
% \end{figure}
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{images/results__IMP__nash_eq_corrected.png}
%     \caption{Average NDR values for different learners in the IMP game. $SQLearner$ agents avoid exploitation by randomising between $H$ and $T$ to obtain a near-optimal NDR value (0) for this game. In contrast to other methods, $SQLearner$ agents have close to zero variance across runs.}
%     \label{fig:results_IMP}
% \end{figure}
$SQLearner$ agents achieve close to perfect cooperation in the IPD (Figure~\ref{fig:results_IPD}).
%We train different learners to play the IPD game. 
% shows the results. 
% For all learners, agents initially defect and move towards an NDR of $-2.0$. 
% This initial bias towards defection is expected, since, for agents trained with random game-play episodes, the benefits of exploitation outweigh the costs of mutual defection. 
Selfish Learner (SL) agents converge to mutually harmful selfish behavior (NDR of $-2.0$). 
Lola-PG agents learn to predict each other's behavior and realize that defection is more likely to lead to mutual harm. 
They subsequently move towards cooperation, but occasionally defect (NDR of $-1.2$). 
$SQLearner$ agents quickly realize the costs of defection, indicated by the small initial dip in the NDR curves.
They subsequently move towards close to 100\% cooperation, with an NDR of $-1.0$.
It is important to note that $SQLearner$ agents have close to zero variance, unlike other methods where the variance in NDR across runs is significant.
%In contrast to other methods, $SQLearner$ agents have close to zero variance across runs.


\textbf{Iterated Matching Pennies (IMP):}
% We train different learners to play the IMP game. 
% The optimal policy for an agent to avoid exploitation is to play $H$ or $T$ perfectly randomly and obtain an NDR of $0$. 
$SQLearner$ agents obtain a near optimal NDR close to $0$ in the IMP (Figure~\ref{fig:results_IMP}). 
Selfish Learner (SL) and Lola-PG agents converge to an exploiter-exploited equilibrium where one agent consistently exploits the other agent. 
This asymmetric exploitation equilibrium is more pronounced for SL agents than for Lola-PG agents. 
As before, we observe that $SQLearner$ agents have close to zero variance across runs, unlike other methods where the variance in NDR is significant.

\textbf{Iterated Chicken Game (ICG):} In the ICG, both $SQLearner$ and LOLA agents obtain an NDR close to $1.0$ (Figure ???). 

\begin{figure}
    \begin{minipage}{0.46\textwidth}
        \centering
        % \includegraphics[width=\linewidth]{images/FINAL--LOLA-SQLoss-on-ICG--ndr.png}
        \includegraphics[width=\linewidth]{images/FINAL--LOLA-SQLoss-on-ICG.png}
        \caption{P(Cooperation) for LOLA and $SQLearner$ agents in ICG. Both agents eventually obtain a near optimal probability of 1.0}
        \label{fig:chicken_game_results}%
    \end{minipage}\hfill%
    
\end{figure}


% \textbf{:} Appendix shows additional results for the iterated Chicken Game.
\begin{figure}[!htb]
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=0.62\linewidth]{images/IPD_results_corrected_final.png}
        \caption{\label{fig:results_IPD}%
        Average NDR values for different learners in IPD. $SQLearner$ agents obtain a near-optimal NDR value $(-1)$ for this game.}
    \end{minipage}\hfill
    \begin{minipage}{0.52\textwidth}
        \centering
        \includegraphics[width=0.92\linewidth]{images/results__IMP__nash_eq_corrected.png}
        \caption{\label{fig:results_IMP}%
        Average NDR values for different learners in IMP. $SQLearner$ agents avoid exploitation by randomising between \textit{H} and \textit{T} to obtain a near-optimal NDR value (0).}
    \end{minipage}\hfill%
\end{figure}%
\begin{figure}[!htb]
    \begin{minipage}{0.38\textwidth}
        \centering
        \includegraphics[width=0.65\linewidth]{images/CoinGame_results_corrected_final_small.png}
        % \includegraphics[width=0.99\linewidth]{images/gamedistill_with_SL_LOLA_SQLoss--final.png}
        % \end{subfigure}~~\\
        % \begin{subfigure}[t]{0.98\linewidth}
        %     \includegraphics[width=\linewidth]{images/100d-feature-vec.png}
        %     \caption{}
        %     \label{fig:feature_vector_plots}%
        % \end{subfigure}
        \caption{\label{fig:coingame_results}%
        Probability that an agent will pick a coin of its color in CoinGame.
        $SQLearner$ agents achieve a cooperation rate close to 1.0 while Lola-PG agents achieve rate close to 0.8.}
        % \textcolor{red}{We start with random oracles at t=0 and as gameplay progresses, \ipdistill develops the clusters effect of which can be seen in the figure on the left.}
        % \textbf{(b)} Representation of clusters obtained after \ipdistill. 
        % Each point is a t-SNE projection of the 100-dimensional feature vector output by the \ipdistill network for an input sequence of states. 
        % The figure on the left is colored based on rewards obtained by the Red and Blue agents. 
        % The figure on the right is colored based on clusters learned by \ipdistill. 
        %\ipdistill correctly identifies two types of state sequences, one for cooperation (blue cluster) and the other for defection (red cluster).
        %See Section~\ref{sec:results:visual-input-gamedistll-and-sqloss} for more details.
        % }%
    \end{minipage}\hfill%
    \begin{minipage}{0.58\textwidth}
        \centering
        \includegraphics[width=0.85\linewidth]{images/gamedistill_with_SL_LOLA_SQLoss--final--final_small.png}
        \caption{\label{fig:gamedistill_oracles_with_lola_and_others}%
        Impact of using pretrained \ipdistill oracles in CoinGame. 
        $SQLearner$ agents (w/ \ipdistill oracles) achieve close to 100\% cooperation. 
        Lola-PG agents eventually (after roughly 4000 epochs) achieve close to 80\% cooperation.
        Interestingly, Lola-PG agents trained w/ \ipdistill oracles converge to higher cooperation rate of 85\% in 300 epochs.}%
    \end{minipage}\hfill%
\end{figure}%

\subsection{Visual Input Games}
\label{sec:results:visual-input-gamedistll-and-sqloss}
% \subsubsection{The Coin Game: GameDistill}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{images/100d-feature-vec.png}
%     \caption{Representation of the clusters learned by \ipdistill. Each point is a t-SNE projection of the 100-dimensional feature vector output by the \ipdistill network for an input sequence of states. The figure on the left is colored based on actual rewards obtained by each agent (Red agent followed by Blue agent). The figure on the right is colored based on clusters learned by \ipdistill. \ipdistill correctly identifies two types of state sequences, one for cooperation (blue cluster) and the other for defection (red cluster).}
%     \label{fig:feature_vector_plots}%
% \end{figure}
% \begin{figure}[t]
%     \centering
%     % \begin{subfigure}[t]{0.4\linewidth}
%     %     \includegraphics[width=\linewidth]{images/results__CoinGame__IPD_formulation.png}
%     %     \caption{Average NDR}
%     %     \label{fig:results_CoinGame_IPD_formulation}
%     % \end{subfigure}\hfil%
%     \begin{subfigure}[t]{\linewidth}
%         \includegraphics[width=\linewidth]{images/CoinGame_results_corrected.png}
%         \caption{
%         Probability of an agent eating a coin of its color
%         }
%         \label{fig:results_CoinGame_probability_of_eating_coin}
%     \end{subfigure}
%     \caption{\label{fig:coingame_results}%
%     Average NDR (a) and cooperation level (b) for learners trained in the Coin Game. 
%     $SQLearner$ agents cooperate (eat only their own coins) to obtain near-optimal NDR (-0.5) in the game. 
%     }
% \end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\linewidth]{images/CoinGame_results_corrected.png}
%     \caption{\label{fig:coingame_results}%
%     Probability of an agent picking a coin of its color for learners trained in the Coin Game. 
%     $SQLearner$ agents cooperate (pick only their own coins) to achieve a near-optimal strategy in the game. 
%     In contrast to Lola-PG, $SQLearner$ agents have close to zero variance across runs. 
%     }
% \end{figure}

$SQLearner$ agents achieve high rates of cooperation in games with visual input (Figure~\ref{fig:coingame_results}).
During game-play, at each step, an agent follows either the action suggested by its cooperation oracle or defection oracle. (Section~\ref{section:approach:social-dilemmas-as-visual-input})
% Further, each $SQLearner$ agent has an additional $SQLoss$ term. 
We compare approaches using the degree of cooperation between agents, measured by the probability that an agent will pick the coin of its color~\cite{foerster2018learning}.
The probability that an $SQLearner$ agent will pick the coin of its color is close to $1.0$. 
This high probability indicates that the other $SQLearner$ agent is cooperating with this agent and only picking coins of its color. 
The probability that a Lola-PG agent will pick a coin of its color is close to $0.8$. 
As expected, the probability of an agent picking its own coin is the smallest for Selfish Learner. 

% Further, $SQLearner$ outperforms LOLA when both  
To evaluate the importance of pre-trained oracles on the performance of $SQLearner$ agents, we compare $SQLearner$ agents to Lola-PG agents trained using the same oracles(
Figure~\ref{fig:gamedistill_oracles_with_lola_and_others}). 
Lola-PG agents with pre-trained oracles converge to a higher cooperation rate ($0.88$) than Lola-PG agents trained directly on visual input but still lower than $SQLearner$ agents.




\begin{comment}

\section{Games with more than 2 players}
\label{sec:beyond_2_players}
Our formulation of $SQLoss$ has the distinct advantage of being fully ego-centric, i.e., the learning agent does not require any information regarding its opponents. This feature enables a straightforward extension of $SQLoss$ beyond the two agent setting, without any change in each agent's learning algorithm. In order to test this extension of $SQLoss$ beyond 2-players, we consider as an example, the problem described in the popular Braess' paradox\cite{Braess1968}, which is a well-known extension of the Prisoner's Dilemma problem to more than 2 agents. We performed additional experiment in this game with 4 agents. We simulated the result when all agents are selfish learners (the $SL$ agent(s)) and also when all agents use $SQLoss$ (the $SQLearner$(s)). We observe that when using selfish learners, all agents converge to Defection and when using $SQLoss$, all agents converge to Cooperation. Detailed explanation of the game, experimental setup and results are shown in Appendix~\ref{appendix:beyond_2_players}. 
% with performance plots for both the 4-player SL agents and 4-player $SQLoss$ agents. 
% To the best of our knowledge, this is the first demonstration of selfish agents learning to cooperate in a sequential social dilemma with more than 2 agents. 
% We need to discuss extension of this to a multi-step (2-step) setting.
% Mainly we need to decide whether to permit asynchronous behavior in that setting or force all vehicles to act synchronously.
\end{comment}


\section{Games with more than 2 players: $SQLoss$ applied to the Braess' Paradox}
\label{section:beyond_2_players}
Our formulation of $SQLoss$ has the distinct advantage of being fully ego-centric, that is, the agent does not require any information regarding its opponents. 
This feature enables a straightforward extension of $SQLoss$ beyond the two agent setting, without any change in each agent's learning algorithm. 
To test this extension of $SQLoss$ beyond 2-players, we consider the problem described in the popular Braess' paradox, which is a well-known extension of the Prisoner's Dilemma problem to more than 2 agents.
\begin{figure}[htb!]
    \begin{minipage}{0.48\textwidth}
        \centering
        % \includegraphics[page=1,width=0.95\linewidth]{images/braess_paradox.pdf}\\
        \includegraphics[page=2,width=0.99\linewidth]{images/braess_paradox.pdf}
        \caption{
        Illustration of Braess' paradox.
        The paradox is concerned with traffic flow from a source ($Start$) to a destination ($End$) with two alternative paths, through two intermediate locations ($A, B$).
        }
        \label{fig:main-paper:braess_paradox}
    \end{minipage}\hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \begin{subfigure}[t]{0.99\linewidth}
            \includegraphics[width=\linewidth]{images/braess_4player_nlpg_summary=10_edited.jpg}
            \caption{Results for 4 NL agents in Braess' Paradox}
            \label{fig:main-paper:braess_4player_nlpg}
        \end{subfigure}~~\\
        \begin{subfigure}[t]{0.99\linewidth}
            \includegraphics[width=\linewidth]{images/braess_4player_sqpg_summary=10_edited.jpg}
            \caption{Results for 4 SQLearner agents in Braess' Paradox}
            \label{fig:main-paper:braess_4player_sqpg}%
        \end{subfigure}%
        \caption{%
            \label{fig:main-paper:braess_results}%
        }%
    \end{minipage}
\end{figure}
% \begin{figure}[htb!]
%     \centering
%     \begin{subfigure}[t]{0.99\linewidth}
%         \includegraphics[width=\linewidth]{images/braess_4player_nlpg_summary=10_edited.jpg}
%         \caption{Results for 4 NL agents in Braess' Environment}
%         \label{fig:braess_4player_nlpg}
%     \end{subfigure}~~\\
%     \begin{subfigure}[t]{0.99\linewidth}
%         \includegraphics[width=\linewidth]{images/braess_4player_sqpg_summary=10_edited.jpg}
%         \caption{Results for 4 SQLearner agents in Braess' Environment}
%         \label{fig:braess_4player_sqpg}%
%     \end{subfigure}%
%     \caption{%
%         \label{fig:braess_results}%
%     }%
% \end{figure}


Fig.~\ref{fig:braess_paradox} illustrates the environment of Braess' paradox.
% The paradox is concerned with traffic flow from a source to a destination with two alternative paths, through two intermediate locations.
% We construct a simplified environment to interpret the policies in the problem given in Braess' paradox as a sequential social dilemma problem. This problem, which we henceforth refer to as the Braess' problem, is concerned with traffic flow from a source to a destination with two alternative paths, through two intermediate locations. This is illustrated in 
Each agent has to travel from the source (Start) to the destination (End) by choosing one of the two paths. 
Each path has two segments separated by the respective intermediate location and the cost of traversing each segment (proportional to the time of travel) is either fixed or is determined based on the number of agents using that segment. 
The cost function is shown in Eq.~\ref{eq:main-paper:braess_cost_function}. 
In the original setup, the two intermediate locations are not connected and each agent has to only choose between one of these paths. 
The equilibrium solution in this case is for half the agents to choose one path and the remaining half the other. 
The modification that leads to the paradox is connecting the two intermediate locations with a cost free directed bridge, thus leading a third possible path for all agents. 
This modification shifts the equilibrium in such a way that all agents now prefer to choose the new path that uses this directed bridge, although this results in a per-agent cost that is higher than each agent's original cost in the absence of this new path. 
This problem has been well studied and the paradox highlights the fact that in strategic settings, increase in the number of available options for all agents, may also lead to decrease in utility for all agents individually and collectively.

We model this problem as a sequential social dilemma, where we define the initial strategy of the agents to choose one of the two original paths as \textit{Cooperation} and the strategy that results in an agent choosing the new path with the directed bridge as \textit{Defection}. 
For simplicity of exposition, we assign integer IDs to agents and define Cooperation for agents with odd-IDs as choosing the path Start-A-End in Fig.~\ref{fig:main-paper:braess_paradox} and Cooperation for agents with even-IDs as choosing the path Start-B-End in Fig~\ref{fig:main-paper:braess_paradox}. 
In this notation, Defection can be defined as an agent choosing the path Start-A-B-End. 
In Figure~\ref{fig:main-paper:braess_paradox} we provide reward numbers, such that the paradox is realized.

\begin{comment}
As described earlier, in this game, Cooperate and Defect have the following interpretation:
\begin{enumerate}
    \item For an odd numbered vehicle – Cooperation implies taking the Start-A-End route.
    \item For an even numbered vehicle – Cooperation implies taking the Start-B-End route (This and above point follow from the assumption that before addition of the new edge A-B, the vehicles were in this equilibrium).
    \item For any vehicle – Defection implies taking the Start-A-B-End route.
\end{enumerate}

\end{comment}

Let $n_{X-Y}$ denote the number of agents using the edge $X-Y$. Then the reward structure for the odd-numbered vehicles (denoted by $R_{odd}$) and the even-numbered vehicles (denoted by $R_{even}$) is computed as shown below.
% \begin{gather*} 
% \end{gather*}%
% \vspace{-15pt}
\begin{equation}%
\label{equation:braess-paradox}
    \begin{split}
        N_{0} &= \text{Total no. of agents}\\
        % R_{var} = 2.0 \\
        R_{0} &= \text{base reward for the agents} = (2.5 * N_{0})/2\\
        R_{odd} &=
        \begin{cases}
          -(n_{Start-A} + n_{B-End}) & \text{if}\ \textit{Defection} \\
          -(n_{Start-A} + R_{0}), & \text{if}\ \textit{Cooperation} \\
        \end{cases}\\
        R_{even} &=
        \begin{cases}
          -(n_{Start-A} + n_{B-End}) & \text{if}\ \textit{Defection} \\
          -(R_{0} + n_{B-End}), & \text{if}\ \textit{Cooperation} \\
        \end{cases}
    \end{split}
    \label{eq:main-paper:braess_cost_function}
\end{equation}
We performed two separate set of experiments in this game with 4 and 6 agents. For each setup, we simulated the result when all agents are selfish learners (the $SL$ agent(s)) and also when all agents use $SQLoss$ (the $SQLearner$(s)). For both these setups, as expected, we observe that when using selfish learners, all agents converge to Defection and when using $SQLoss$, all agents converge to Cooperation. We present the results for the Braess' Paradox experiment in Figure~\ref{fig:main-papbraess_results}.

Figure~\ref{fig:main-paper:braess_4player_sqpg} shows the results for 4 SL-agents playing in the environment. 
It is clear that if 4 SL agents play in the environment, then they eventually end up defecting i.e. $\lim_{E \to \infty}\mathbb{P}(Cooperation) \to 0$, where $E$ denotes the epoch. 
Figure~\ref{fig:main-paper:braess_4player_sqpg} illustrates the behaviour of the $SQLearner$ agents. 
The SQLearner agents eventually learn to cooperate and thus the $\lim_{E \to \infty}\mathbb{P}(Cooperation) \to 1$. To the best of our knowledge, this is the first demonstration of independent agents learning to cooperate in a sequential social dilemma with more than 2 agents. 

\section{$SQLoss$: Similarities to Popular Hand-Crafted Strategies}

\section{Limitations of $SQLoss$}



==> rebuttal.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

% \section*{ICML - Author Response}


\section{\ipdistill}
\label{appendix:gamedistill-explanation}
\ipdistill need not have the same information constraints like $SQLoss$. \ipdistill additionally requires the rewards obtained by the opponent as well to perform effective clustering of trajectory embeddings while $SQLoss$ does not require the opponent's rewards. We consider games that are fair to both the agents and this results in symmetric rewards for both the agents. In such games with symmetric rewards, its fair to assume that the rewards of both the agents are visible to an agent. To justify this, we can also imagine the scenario where the agent plays an hypothetical game-play that mimics the opponent to obtain the rewards of the opponent. We thus posit that having the opponent's rewards during training \ipdistill does not require any extra information. In games with asymmetric rewards, a lot of questions remain unanswered in the literature.

Each episode contains the sequence of states, actions, and rewards for both agents. 

For instance, Figure~\ref{fig:oracle_predictions} (Appendix~\ref{appendix:oracle:illustration}) illustrates the cooperation and defection oracles extracted by the Red agent using \ipdistill in the Coin Game.



\section{Reward modifications needed to make this work with Q-learning}
\begin{enumerate}
    \item In state CC, for example, if you take D, you get the normal next state reward, however, if you take C, SQLoss kicks in to give the extra SQLoss reward.
    \item For CD, SQLoss kicks in for C
    \item For DC, SQLoss kicks in for D
    \item For DD, SQLoss kicks in for D
    So, interestingly, every time you stick to the status quo, you get this extra reward term, otherwise you do not 
\end{enumerate}

\section{extra stuff}

Therefore, $\pi^{1} (C|CC) < \pi^{1} (D|CC)$ post the update. 

Note that $\pi (u_{t}|s_{t})$ For $s_{t}=CC$, $u_{t-1}^{1}=C$ and $\hat R_{t}^{1}(\hat \uptau_1) << 0$.

Initially, $\pi^{1} (u_{t}^{1}|s_{t})$ is random. 
Consider a gradient update to $\pi^{1}$ using only the $SQLoss$ term from Equation 7.

Therefore, $\pi^{1} (C|CC) < \pi^{1} (D|CC)$ post the update. 
Similarly, $\pi^{1} (D|DD) < \pi^{1} (C|DD)$.
For $s_{t}=CD, u_{t-1}^{1}=C$ and $\hat R_{t}^{1}(\hat \uptau_1) << 0$.
Therefore, $\pi^{1} (C|CD) < \pi^{1} (D|CD)$. 
Note that, for $s_{t}=DC, u_{t-1}^{1}=D$ and $\hat R_{t}^{1}(\hat \uptau_1) = 0$. 
Therefore, $\pi^{1} (D|DC) > \pi^{1} (C|DC)$. 

If we use \textbf{only} $SQLoss$ gradient updates, and $s_0=CC$, then both agents play $D$ (since $\pi^{1} (C|CC) < \pi^{1} (D|CC)$) to reach $s_1=DD$.
In $s_1=DD$ both agents play $C$ to reach $s_2=CC$ and this $[CC,DD]$ sequence oscillates.
If $s_0=DC$, then agent 1 plays $D$, and agent 2 plays $C$ (for agent 2 the state is $CD$) to reach $s_1=DD$ and subsequently a $[DD,CC]$ sequence. 
The same is true for $s_0=CD$.
Hence, regardless of $s_0$, using \textbf{only} $SQLoss$ leads to a $[CC,DD]$ sequence (intuition is described in section 2.3.1).


In the absence of $SQLoss$, consider policy $\pi^{1} (u_{t}^{1}|s_{t})$, which is initially random.
After playing a certain number of games against 
$\pi^{2} (u_{t}^{2}|s_{t})$ (also random), let $E^{1}(u_{t}|s_{t})$ denote the expected reward when playing $u_{t}$ in $s_{t}$.
$E^{1}(C|CC)=0.5(-1) + V(CC) + 0.5(-3) + V(CD)=-2 + V(CD) + V(CC)$ (If $a_{1}$ plays C, then with $p=0.5$ it stays in CC, with $p=0.5$ it goes to CD, and $r_{t}$ denotes the reward of subsequent random play).
Similarly, $E^{1}(D|CC)=0.5(0) + V(DC) + 0.5(-2) + V(DD)=-1 + V(DC) + V(DD)$.
Therefore, $E^{1}(D|CC) > E^{1}(C|CC)$.
Also, $E^{1}(C|DC)=0.5(-1)+ V(CC) + 0.5(-3) + V(CD)=-2 + V(CC) + V(CD)$, $E^{1}(D|DC)=0.5(0) + V(DC) + 0.5(-2) + V(DD)=-1 + V(DC) + V(DD)$.
Therefore, $E^{1}(D|DC) > E^{1}(C|DC)$.
Similarly, $E^{1}(D|CD) > E^{1}(C|CD)$ and $E^{1}(D|DD) > E^{1}(C|DD)$.
Note that for random agents, $V(CC)=V(DD)=V(DC)=V(CD)$.
After the gradient update $\pi^{1} (D|s_{t}) > \pi^{1} (C|s_{t})$ and $\pi^{2} (D|s_{t}) > \pi^{2} (C|s_{t})$.
As agents learn, $V(DD) \xrightarrow{} -2$, $V(CC) \xrightarrow{} -3$, because cooperative agents are exploited. 
Therefore, $a_{1}$ and $a_{2}$ converge to mutual defection. 


However, with the $SQLoss$ term, $E^{1}(C|CC)=-2 + V(CD) + V(CC) + \kappa*(-1)$.
Also, $E^{1}(D|DD)=-1 + V(DD) + V(DC) + \kappa*(-2)$.
$E^{1}(C|CD)=-2 + V(CD) + V(CC) + \kappa*(-3)$.
$E^{1}(D|DC)=-1 + V(DC) + V(DD) + \kappa*(0)$.
As before, for random agents, $V(CC)=V(DD)=V(DC)=V(CD)$.
The key idea is that with the addition of $SQLoss$, $E^{1}(C|DD) > E^{1}(D|DD)$.
Now, to achieve cooperation, we need $E^{1}(C|CC) > E^{1}(D|CC)$.
$E^{1}(C|CC)=-2 + V(CD) + V(CC) + \kappa*(-1)$.
$E^{1}(D|CC)=-1 + V(DC) + V(DD)$.
Since $\pi^{1} (D|CD) > \pi^{1} (C|CD)$ and $\pi^{1} (D|DC) > \pi^{1} (C|DC)$, over time $V(CD) V(CD) V(DD)$  

Therefore, $a_{1}$ and $a_{2}$ initially move to a $[CC,DD]$ sequence. 



pushes agents in the IPD towards either $CC$ or $DD$.
In the absence of $SQLoss$, the IPD reward $R_{t}^{1}(\uptau_1)$ (Equation 5) pushes agents individually towards $DC$, and therefore leads to mutual defection. 
However, with $SQLoss$, $DC$ is diminished, $[DD,CC]$ remain and the IPD reward moves agents towards $CC$ since $R_{t}(CC) > R_{t}(CC)$.



However, with the $SQLoss$ term pushes agents in the IPD towards either $CC$ or $DD$.
In the absence of $SQLoss$, the IPD reward $R_{t}^{1}(\uptau_1)$ (Equation 5) pushes agents individually towards $DC$, and therefore leads to mutual defection. 
However, with $SQLoss$, $DC$ is diminished, $[DD,CC]$ remain and the IPD reward moves agents towards $CC$ since $R_{t}(CC) > R_{t}(CC)$.



\section*{0. $SQLoss$: Shortened Theory}
Equation 6 describes the standard policy gradient. 
The $log\pi^{1} (u_{t}^{1}|s_{t})$ term maximises the likelihood of reproducing the training trajectories.
The return term pulls down trajectories that have poor return.
The overall effect is to reproduce trajectories that have high returns. 

Lemma 1:
For agents trained with random exploration in the IPD, $Q_{\pi}(D|s_t) > Q_{\pi}(C|s_t)$ for all $s_t$
Let $Q_{\pi}(a_t|s_t)$ denote the expected return of taking $a_t$ in $s_t$.
Let $V_{\pi}(s_t)$ denote the expected return from state $s_t$.
$Q_{\pi}(C|CC)=-2 + 0.5[V_{\pi}(CC) + V_{\pi}(CD)]$
$Q_{\pi}(D|CC)=-1 + 0.5[V_{\pi}(DC) + V_{\pi}(DD)]$
And similarly for other states.
Since $V_{\pi}(CC)=V_{\pi}(CD)=V_{\pi}(DC)=V_{\pi}(DD)$ for randomly playing agents, $Q_{\pi}(D|s_t) > Q_{\pi}(C|s_t)$ for all $s_t$.

Lemma 2:
Agents trained to only maximise the expected reward in IPD will converge to mutual defection. 

This lemma follows from Lemma~\ref{lemma:random:agents:like:D}.
Agents initially collect trajectories from random exploration. 
They use these trajectories to learn a policy that optimises for long-term return. 
These learned policies always play $D$ as described in Lemma~\ref{lemma:random:agents:like:D}.

Equation 7 describes the gradient for $SQLoss$. The $log\pi^{1} (u_{t-1}^{1}|s_{t})$ term maximises the likelihood of taking $u_{t-1}$ in $s_{t}$.
The imagined episode return term pulls down trajectories that have poor imagined return. 

Lemma 3:
Agents trained on random trajectories using only $SQLoss$ oscillate between $CC$ and $DD$. 

For IPD, $s_{t} = (u_{t-1}^{1}, u_{t-1}^{2})$.
Consider state $CC$, with $u_{t-1}^{1}=C$.
$\pi^{1} (D|CC)$ is randomly initialised. 
The $SQLoss$ term reduces the likelihood of $\pi^{1} (C|CC)$ because $\hat R_{t}(\hat \uptau_1) < 0$. 
Therefore, $\pi^{1} (D|CC) > \pi^{1} (C|CC)$.

Similarly, for $CD$, the $SQLoss$ term reduces the likelihood of $\pi^{1} (C|CD)$.
Therefore, $\pi^{1} (D|CD) > \pi^{1} (C|CD)$.
For $DC$, $\hat R_{t}(\hat \uptau_1) = 0$, therefore $\pi^{1} (D|DC) > \pi^{1} (C|DC)$.
Interestingly, for $DD$, the $SQLoss$ term reduces the likelihood of $\pi^{1} (D|DD)$ and therefore $\pi^{1} (C|DD) > \pi^{1} (D|DD)$. 

Now, if $s_t$ is $CC$ or $DD$, then $s_{t+1}$ is $DD$ or $CC$ and these states oscillate. 
If $s_t$ is $CD$ or $DC$, then $s_{t+1}$ is $DD$, $s_{t+2}$ is $CC$ and again $CC$ and $DD$ oscillate. 
This oscillation is key to the emergence of cooperation as explained in section 2.3.1.

Lemma 4:
For agents trained using both standard loss and $SQLoss$, $\pi (C|CC) > \pi^{1} (D|CC)$.


For $CD$, $DC$, both the standard loss and $SQLoss$ push the policy towards $D$.
For $DD$, with sufficiently high $\kappa$ (as shown in our experiments), the $SQLoss$ term overcomes the standard loss and pushes the agent towards $C$.
For $CC$, initially both the standard loss and $SQLoss$ push the policy towards $D$.
However, as training progresses, the incidence of $CD$ and $DC$ diminish because of $SQLoss$ as described in Lemma 3.
Therefore, $V_{\pi}(CD) \approx V_{\pi}(DC)$ since agents immediately move from both states to $DD$. 
Intuitively, agents lose the opportunity to exploit the other agent. 
In equation 9, with $V_{\pi}(CD) \approx V_{\pi}(DC)$, $Q_{\pi}(C|CC) > Q_{\pi}(D|CC)$ and the standard loss pushes the policy so that $\pi (C|CC) > \pi (D|CC)$. 
Once this happens, agents converge to mutual cooperation.

We have truncated the complete proof for space constraints. 

% \section{GameDistill: Pseudo-Code}

% \begin{algorithm*}
% \caption{Calculate $y = x^n$}
% \begin{algorithmic}
% % \REQUIRE $n \geq 0 \vee x \neq 0$
% \ENSURE $y = x^n$
% \STATE $y \leftarrow 1$

% 1. Collect list of episodes(Eps) with (r1,r2) $\gt$ 0 from random game play

% 2. \FORALL{agents}
%     a. Create dataset\newline
%     $listEpisodes, myRewards, opponentRewards, gameAttrs \leftarrow [~], [~], [~], [~]$ \newline
%     \FOR{episode in Eps}
%         \item\FOR{(s,a,r,s’) in episode}
%             if r\gt0, then add sequence of last three states leading up to s’ to listEpisodes, add respective rewards to myRewards and opponentRewards, add color of coin to gameAttrs 
%         \ENDFOR
%         $inp_ep=listEpisodes.reshape([batch*4,3, inSize]) $
%         $(inSize=[7x7] for stag_hunt,[3x3] for coingame) $
%     \ENDFOR
%     b. Train Sequence Encoding Network: 
%         trnk= (Net[Conv(3x3,64),Relu,Conv(3x3,64),Relu,Conv(3x3,64),Relu]).reshape(batch,-1) 
%         baseNet=Net[trnk(),fc(100),relu,fc(10),relu] 
%         Cnet= Net[baseNet,fc(100),fc(2)] 
%         SRnet= Net[baseNet,fc(100),fc(1)] 
%         ORnet= Net[baseNet,fc(100),fc(1)] 
    
%         Train with NetLoss=BCE(Cnet(inp_ep) , gameAttrs) + MSE(SRnet(inp_ep), my_rewards) + MSE(ORnet(inp_ep), oppRewards), AdamOptimizer, lr=3e-3, epochs=200 
%     c. Embeddings=[(episode,baseNet(episode)) for episode in list_episodes]  
%     d. Cluster embeddings using Agglomerative Clustering[1], numClusters=2  
%     e. Map episode to clusters from step d 
%     e. Train oracle for each cluster  
%         Onet=Net[Conv(2x2,128),Relu,Conv(2x2,128),Relu,Conv(2x2,64),Relu,fc(128),Relu,fc(4),SoftMax]for eps in episodes: 
%             for st, act in eps 
%                 Train Onet with loss 
%                 CE(Onet (st), act) and SGD, lr=1e-2 

%     \ENDFOR
% \end{algorithmic}
% \end{algorithm*}


